Token-based Vehicular Security System (TVSS): Scalable, Secure, Low-latency Public Key Infrastructure for Connected Vehicles

Connected and Autonomous vehicles stand to drastically improve the safety and efficiency of the transportation system in the near future while also reducing pollution. These systems leverage communication to coordinate among vehicles and infrastructure in service of a number of safety and efficiency driver assist and even fully autonomous applications. Attackers can compromise these systems in a number of ways including by falsifying communication messages, making it critical to support security mechanisms that can operate and scale in dynamic scenarios. Towards this end, we present TVSS, a new VPKI system which improves drastically over prior work in the area (including over SCMS; the US department of transportation standard for VPKI). TVSS leverages the idea of unforgeable tokens to enable rapid verification at the road side units (RSUs), which are part of the road infrastructure at the edge of the network. This edge based solution enables agile authentication by avoiding the need for back-end servers during the potentially short contact time between a moving vehicle and the infrastructure. It also results in several security advantages: (1) Scalable Revocation: it greatly simplifies the revocation problem, a difficult problem in large scale certificate systems; and (2) Faster Refresh: Vehicles interact more frequently with the system to refresh their credentials, improving the privacy of the system. We provide a construction of the system and formally prove its security. Field experiments on a test-bed we develop consisting of on-board units (OBUs) and RSUs shows substantial reduction in the latency of refreshing credentials compared to SCMS, allowing the system to work even with smaller window of connectivity when vehicles are moving at higher speeds. Notably, we are able to execute the bottleneck operation of our scheme with a stationary RSU while traveling at highway speeds .

==> background_scms.tex <==
\section{Background}
\label{sec:background}

The Security Credential Management System (SCMS) was originally developed and published by \cite{Brecht2018SCMS} and adopted by the USDOT as the official vehicle's VPKI for future applications of connected and autonomous vehicles \cite{USDOTSCMS}. As we will see in the related work in Section \ref{sec:related}, there is little exposure on the SCMS by the research community despite the fact that this system has been officially adopted by a government agency. Since our work in this paper will focus on the USDOT assumptions and requirements, in this section, we will define the general requirement of the USDOT VPKI system then provide a brief background on the USDOT adopted VPKI, the SCMS. Finally, we will provide a comparative analysis between SCMS and our system, DVSS. Figure~\ref{fig:scms and dvss arch} shows an overview of the SCMS and DVSS architecture. Readers who are not familiar with the cryptography used in this paper is urged to look at Appendix~\ref{sec:crypto prelim}.

\subsection{VPKI Requirements}

\textbf{1- Anonymity:} Typically in a PKI security paradigm, a sender of a message authenticate its messages by applying a digital signature to every message he/she sends out where the identity of the signer is endorsed by a digital certificate that is signed by a trusted third party known as a Certification Authority (CA). However in a VPKI security paradigm, having identifying information in messages sent out by vehicles would expose the privacy of drivers; the digital certificate of the vehicle might include the driver's name or a license number. A simple mitigation to such problem is replacing the identifying information in the digital certificate with a pseudonym one. This type of certification is commonly known as a pseudonym certificate (PC) and its main objective is to preserve the \emph{anonymity} of its user from the public while authenticate the legitimacy of the message signer during its participation in the VPKI system.

\textbf{2- Unlinkability:} If a vehicle is assigned a single PC, any public entity can track that vehicle by matching signatures from the vehicle's messages which are signed by the same PC. In other words, a malicious party can track a vehicle across different times and locations via PC signatures and eventually build a profile of the victim vehicle which might partially reveal the identity of the driver (e.g. driving patterns of a daily commute). Therefore, the VPKI system should allow the vehicle to periodically switch between multiple PCs to prevent vehicle tracking. This requirement is known as \emph{unlinkability} which means no public entity should be able to link two or more PCs to the same user. Under this definition, we can describe unlinkability as a conservative form of anonymity (compromising unlinkability leads to compromising anonymity).

\textbf{3- Unlinkability from VPKI Administrators:} The previous two requirements (1 and 2) are established against public entities (outsiders) and not the VPKI system itself (insiders). In other words, drivers might be hesitant to participate in such system knowing that every single vehicular trip they make is being monitored by the VPKI system since it is the very system who provisioned their vehicles with PCs in the first place. Therefore to extend the unlinkability of vehicles to the fullest, the VPKI system should also not be able to reveal the true identity of a PC owner or link multiple PCs to the same owner.

\textbf{4- Revocability:} In case a vehicle misbehaves (e.g. sending out maliciously crafted messages), the VPKI system should have the capability to reveal the true identity of the misbehaving vehicle from its PC for revocation and accountability. Note that requirement 3 might be interpreted as complete unlinkability which conflicts with requirement 4. Therefore, a middle ground between requirement 3 and 4 must be established which dictates that \emph{no single VPKI entity should have the privilege to reveal a vehicle's identity or track multiple PCs to the same vehicle}. In other words, in order for the VPKI system to reveal a vehicle identity, multiple VPKI entities must cooperate together in order to complete the revocation task. The division-of-labor scheme for vehicle revocation is adopted to prevent -for example- a curious system admin from single-handedly revealing and tracking VPKI vehicles.

% \begin{figure*}[h]
% % \vspace{-5pt}
% \centering 
% \includegraphics[width=.9\linewidth,keepaspectratio]{Images/SCMS overview 3.png}
% % \vspace{-6pt}
% \caption{SCMS Architecture Overview~\cite{CV2019USDOT}.}
% % \ahmed{Is this your diagram?} \abdulrahman{this diagram is brought from the SCMS conference paper}
% \label{fig:scms overview}
% % \vspace{-12pt}
% \end{figure*}

% \subsection{Main Functions}
\subsection{SCMS Overview}

% The following commented paragraph is the short version of "SCMS Overview"

% Before a vehicle participate in the SCMS, it must obtain a long-term certificate, called Enrollment Certificate (EC), signed by an Enrollment Certification Authority (ECA). All messages sent by the vehicle to the SCMS must be signed by its EC. Once a vehicle owns an EC (which only happens once for each new vehicle or vehicle ownership transfer), the vehicle can request multiple Pseudonym Certificates (PC) from an SCMS entity called Pseudonym Certification Authority (PCA). The PCs are then used to communicate securely and \emph{anonymously} with other vehicles while the sending vehicle keeps swapping between PCs (e.g. every 5 minutes) to preserve \emph{unlinkability}. Note that in figure \ref{fig:scms and dvss arch} all SCMS certification entities are consolidated in "Certificate Authority (CA)". The suggested SCMS parameters allow a vehicle to have 20 to 40 PCs that are simultaneously valid for one week. All PC requests are sent to an SCMS entity called Registration Authority (RA) that validates, processes, and forwards requests for PCs to the PCA. The division-of-labor between PCA and RA is to satisfy requirement 3 and 4. Furthermore, to preserve the vehicles' location anonymity, all vehicles' messages to the SCMS are tunneled through an SCMS gateway called Location Obscurer Proxy (LOP) which has the role of obscuring the vehicle's location (i.e. IP address) by sending the vehicle's messages on its behalf to the desired SCMS destination server. In case of a vehicle misbehavior incident, the Misbehavior Authority (MA) is the SCMS entity responsible of initiating the revocation process among the other SCMS entities with the support of Linkage Authority 1 (LA1) and Linkage Authority 2 (LA2). LA1 and LA2 store a hash chain for each vehicle where each value in the hash can be used by the MA to reveal a vehicle identity. The division-of-labor between two Linkage Authorities is implemented to prevent a single authority from unlawfully revealing the identities of vehicles.

In this subsection, we provide a high-level overview of the the main functions in SCMS. The details of each function is explained in detail in the next subsections.

\vskip3mm\noindent\textbf{Device Bootstrapping:} The main goal of the SCMS is distributing digital certificates to vehicles for secure and privacy-preserved communications among the vehicles themselves and between the vehicles and the SCMS backend system. The first step for any vehicle joining the system is obtaining a long-term certificate, called Enrollment Certificate (EC), signed by an Enrollment Certification Authority (ECA), as well as other important information such as public certificates of several SCMS authorities. A vehicle's EC acts as a passport that allows the vehicle to send authenticated service requests to the SCMS backend

\vskip3mm\noindent\textbf{Pseudonym Certificate Provisioning:} Once a vehicle owns an EC (which only happens once for each new vehicle or vehicle ownership transfer), the vehicle can request multiple Pseudonym Certificates (PC) and sign that request using its EC. The main purpose of PCs is to allow vehicles to communicate securely and anonymously among each other by swapping between PCs (e.g. every 5 minutes) in order to prevent an observer from tracking a vehicle by observing the same certificate signatures across two or more different locations. The current SCMS parameters allow a vehicle to have 20 to 40 PCs that are simultaneously valid for one week. All PC requests are sent to an SCMS entity called Registration Authority (RA) that validates, processes, and forwards requests for PCs to a Pseudonym Certification Authority (PCA). The PC provisioning process is described in details in Section \ref{sub:pc_provisioning}

\vskip3mm\noindent\textbf{Preserving Anonymity \& Unlinkability:}
From the PC provisioning process described above, one can see that the process of creating PCs is divided between two separate SCMS entities, RA and PCA. The main reason of this design is to prevent a single SCMS entity from linking the actual vehicle's identity (i.e. EC) to its corresponding PCs (\emph{anonymity}). In other words, the PCA cannot tell which of the PCs it has created belong to which vehicle since the requests are coming from the RA. Likewise, the RA cannot peek into the PCs (encrypted with the vehicle's public key) when it forwards the PCs to the vehicle. Furthermore, the RA shuffles the PC requests before sending it to the PCA to prevent the PCA from determining if two or more PCs belong to the same vehicle (\emph{unlinkability}). To preserve the vehicles' location anonymity, whenever a vehicle needs to communicate with the backend system, it communicates via an SCMS gateway called Location Obscurer Proxy (LOP) which has the role of obscuring the vehicle's location (i.e. IP address) by sending the vehicle's messages on its behalf to the desired SCMS destination server.



\vskip3mm\noindent\textbf{Misbehavior Reporting \& Certificate Revocation:} In case a vehicle is misbehaving (e.g. sending falsified information), other vehicles report this misbehavior to an SCMS entity called Misbehavior Authority (MA) and include the misbehaving vehicle's PC in the report. Once the misbehavior has been proven, the MA revokes all the currently active PCs of the vehicle by adding them in a Certificate Revocation List (CRL) to warn other vehicles from dealing with the culprit vehicle. The MA also adds the vehicle's corresponding EC in an internal EC Blacklist ($\BL$) that is only accessible by SCMS entities to prevent future PC requests from the blacklisted vehicle. The process of linking the PCs with its corresponding EC takes place among several entities and it is described in Section ~\ref{sub:scms_revocation}.


\subsection{Pseudonym Certificates Provisioning Process}
\label{sub:pc_provisioning}

When a vehicle wants to obtain a PC, it sends a PC request signed by its corresponding EC to the SCMS backend system via an RSU. First, the vehicle creates a PC public/private keypair $(g^x, x)$ and a session public/private keypair $(g^y, y)$. Then, the vehicle creates a PC request, attaches $g^x$ and $g^y$, signs it with its EC, then sends it to the backend system. The request is then relayed from the RSU to the RA via the LOP to hide the vehicle's location. Then for each PC request, the RA creates two sets of 20 random numbers \cut{$r_{i} \in $}$\{r_{1},\cdots, r_{20}\}$ and \cut{$r'_{j} \in $}$\{r'_{1},\cdots, r'_{20}\}$ (assuming the SCMS is configured to generate 20 PCs per request). The RA then raises $g^x$ to each $r_{i}$ and $g^y$ to each $r'_{i}$ for all ${i=1, \cdots, 20}$, creating 2 sets of 20 different public keys each, $\{g^{x.r_{i}}\}_i$ and $\{g^{y.r'_{i}}\}_i$; this process is known as Butterfly Key Expansion and its main purpose is to offload the creation of the 20 public keys to the RA (without knowledge of corresponding private keys) which reduces vehicle uplink bandwidth. After that, the RA sends each pair of ($g^{x.r_{i}}, g^{y.r'_{i}}$) to the PCA. Note that to preserve the unlinkability requirement, the RA shuffles between the pairs from different vehicles' requests before sending them to the PCA. This prevents the PCA from linking a group of keypairs (and ultimately PCs) to the same vehicle since PCA (according to the discrete log assumption) cannot distinguish if $g^{x.r_{i}},g^{x.r_{j}}$ are generated from the same PC request. The PCA then creates a random number $\hat r_{i}$ for each $g^{x.r_{i}}$ and raises it to that random number and signs the newly created PC public key using the PCA's private key, creating a PC$ = (g^{x.r_{i}.\hat r_{i}}, \sigma)$. The process of raising $g^{x.r_{i}}$ to a new random number $\hat r_{i}$ by the PCA is done to prevent the RA from linking multiple PCs to the same vehicle (preserving unlinkability) since the RA is the SCMS entity who performed the Butterfly Key Expansion process. It also prevents the RA from linking a PC to its corresponding EC (preserving anonymity) since it knows who is the requesting vehicle. After that, the PCA encrypts $\ct = $(PC, $\hat r_{i}$) using its paired $g^{y.r'_{i}}$ (which is received from the RA) and sends it back to the RA. Finally, the RA sends the newly signed PCs to the requesting vehicle by relying  $\{\ct, r_{i}, r'_{i}\}$ over a secure channel (\eg TLS). Note that the PCA and RA keep a \emph{request reference number} for each keypair in order for the RA to know which signed PC to send to which vehicle without the need of looking into the encrypted content of $\ct$. Upon receiving the response from the RA, the vehicle computes the expanded private key of each $g^{y.r'_{i}}$ as $y.r'_{i}$ and decrypt the PCA messages. It then computes the expanded private keys of each PC, $g^{x.r_{i}.\hat r_{i}}$ as $x.r_{i}.\hat r_{i}$.

\subsection{Enrollment \& Pseudonym Certificate Revocation Process}
\label{sub:scms_revocation}

\vskip3mm \noindent\textbf{Creating Linkability:} If a vehicle misbehaves, the SCMS should be able to link the vehicle's PC to its EC for revocation and accountability. 
% The PC provisioning process described in the previous section provides complete unlinkability even if all SCMS entities cooperate together (which is undesirable).
Naively, all non-expired PCs of a single revoked vehicle are added to the pseudonym certificate revocation list (PCRL) upon revocation; however, the PCRL size becomes extremely large and bandwidth consuming since SCMS generates a large number of PCs per vehicle. In order to have a fixed number of entries (namely one entry) required to be added in the PCRL per revoked vehicle regardless of the number of revoked PCs, SCMS links all PCs of  a single vehicle in such a way that no single entity in the system is able to distinguish their relation (and thus acheive unlinkability). To provide linkability of misbehaving vehicles, a Linkage Value $LV$ (\ie a PC id) is added to each $PC$ created by the PCA.

To create the $LV$, two SCMS entities are responsible for this task, called Linkage Authority 1 ($LA_{1}$) and Linkage Authority 2 ($LA_{2}$). For each newly created $EC$, each $LA$ creates and assigns a random number for that $EC$ called Linkage Seed 0 ($LS_{0}$) which will be used to create a hash chain of Linkage Seeds $LS_{i}$ such that $LS_{i+1} = H(LS_{i})$. Each $LS_{i}$ acts as a reference value for a batch of 20 $PCs$. The $LS_{i}$ is then used to create 20 different values called Prelinkage Values $PV_{j} \in (PV_{1},...,PV_{20})$ using an AES function such as $PV_{j} = \enc_{LS_{i}} (j||LA_{ID})$ where $LA_{ID}$ is the ID of the $LA$ which is used to prevent the chance of having the two $LAs$ randomly choose the same $LS_{0}$ seed for the same vehicle. Finally, each $PV_{j}$ from $LA_{1}$ and $LA_{2}$ for a given batch $LS_{i}$ are XORed together creating $LV_{i,j}$ ($LV$ for PC $j$ from batch number $i$). Notice that the creation of a single $LV$ is divided between two $LAs$ to prevent a single LA from linking multiple $PCs$ by simply looking at their $LVs$. Also, the PCA cannot retrieve  the two corresponding $LS_i$ given the two $PV_j$ only because it does not know the AES key (\ie $LS_i$). Furthermore, the XORing operation of the two $PV_{j}$ is done by the $PCA$ during the $PC$ creation process. Note that since the PCA does not know the EC of the requesting vehicle, the LAs cannot determine from which $LS_{0}$ seed the $PV$ should be derived from since the PCA cannot provide the EC to them. Therefore, the $PV$ request is done by the RA during the key expansion process (since it is the entity who knows the EC of the requesting vehicle and the batch number $i$) and passes it to the PCA. Furthermore, to prevent the RA from linking PCs to the same vehicle via their $LVs$ (by XORing its $PVs$), LAs encrypt the $PVs$ with the PCA's public key before passing them to the RA.

\vskip3mm \noindent\textbf{Revoking a Misbehaving Vehicle's Certificate:} Once a vehicle is determined to be misbehaving, the MA contacts the PCA and requests the 'PC request reference number' between the PCA and the RA that was used to create the misbehaving PC. Based on reference number, the MA instructs the RA to add the EC of the vehicle who requested the PC, to an SCMS internal blacklist (\BL) in order to prevent future PC provisioning requests from the misbehaving vehicle. Then the MA (with the help of RA) instructs the two LAs to reveal their $LS_{i}$ for the blacklisted EC (via EC initial seed $LS_{0}$) for a given batch $i$. Assuming the SCMS is configured to allow a vehicle to have 20 $PCs$ every week, each $LS_{i}$ represents the linkage seed of week $i$ for a vehicle. In other words, based on the validity time of a given PC, the batch number is inferred from the week number. After that, the two LAs add the $LS_{i}$ of the misbehaving vehicle to a public PCRL. Once the two $LS_{i}$ are made public, any vehicle can compute all subsequent $LS_{i+1}$, derive the $PV$ for week $i$, and XOR the $LVs$ of the misbehaving vehicle for all subsequent weeks until the vehicle's EC expiration date (or simply until the end of the current week since the misbehaving vehicle is blacklisted from any future PCs).

\subsection{Comparative Analysis Between DVSS \& SCMS}

\vskip3mm \noindent\textbf{Simple Architectural Design:} The design of the DVSS is far simpler than of the SCMS's which makes our system easier to maintain and extend with additional functionalities without risking a cascade of changes across other system's components. As discussed in section \ref{sec:background}, the SCMS requires multiple entities with complex relationships among them to preserve the anonymity and unlinkability of vehicles. On the other hand, DVSS enables vehicles to acquire PCs in two simple phases, tokens acquisition phase, $\tokengen$, (a vehicle requests a set of tokens from the DVSS backend system before the start of the trip such as when the vehicle is parked at night), and PC provisioning phase, $\pseudogen$, (a vehicle provides an RSU with a token in exchange for a new PC). Importantly, each phase requires communication with a single system entity. With this simple -yet effective- VPKI design, the anonymity, unlinkability, and revocability of vehicles are preserved without complex interactions between system entities. For instance, if the SCMS decided to follow our design and push the PC provisioning to the RSUs, this would put the RSUs (and ultimately the anonymity and unlinkability of vehicles) at risk since RSUs are physically accessible to malicious parties and any compromised RSU would potentially compromise the security of the system. In DVSS, compromised RSUs won't reveal any identifying information to the attacker since the tokens received by the RSUs are anonymous by design.

\vskip3mm \noindent\textbf{No Sybil Attack:} The SCMS allows a vehicle to hold onto multiple PCs that are simultaneously valid at the same time. This enables a misbehaving vehicle to launch what is known as Sybil Attack where the misbehaving vehicle communicates with other vehicles/RSU with multiple identities. This attack could -for example- give the impression of a congested road or intersection which might influence the behavior of other vehicles/RSUs such as a smart intersection controller to extend the green light of the congested intersection lane where the attacker resides. On the other hand, a vehicle under the DVSS can hold onto multiple tokens, each with a non-overlapping validity period. In other words, a vehicle can request multiple PCs with multiple tokens but each PC will have a validity period that is different from the rest of the PCs. If a misbehaving vehicle tries to request multiple PCs from different RSUs simultaneously, each PC can only be used in a unique region, which makes Sybil attacks unfeasible; this particular case however causes clone attacks, which our system handles as will be shown later.

\vskip3mm \noindent\textbf{Short PCRLs:} As discussed in Section~\ref{sec:intro}, the size of a PCRL in SCMS is $N\times |V'|$ where $N$ is the number of active PCs per vehicle and $|V'|$ is the number of revoked vehicles. If we assume 1\% of the US vehicles are revoked, and the SCMS allows a vehicle to have 20 simultaneously active PCs, then the number of entries in the PCRL that each vehicle must maintain is 70 millions which is not very scalable for a vehicular network; likewise, the PCRL requires high bandwidth because of its large size even after utilization of the hash chain mechanism (\ie PCRL would have 3,500,000 entries). A possible solution is confining the validity of PCs within a predefined geographical area where each area has its own PCRL. However, adding a validity-location attribute to a PC in SCMS would violate the unlinkability of vehicles
% , either by RA or PCA
by PCA or anonymity by RA
(depending on the design choice of who the location handler is). Another mitigating approach (which is suggested by the SCMS) is dividing the PCRL into multiple PCRLs based on some attribute such as the region of misbehavior. However, since a vehicle could have a week-worth of PCs, a misbehaving vehicle might travel outside the regional PCRL and remain unrevoked in neighboring regions. In DVSS, each RSU is responsible for providing PCs within its region. Therefore, it is possible for an RSU to issue a PC that is confined within its region of control without violating the unlinkability of vehicles since the linkability information is embedded with the tokens (which is provided by the DVSS CA), not the PCs. In other words, the CA can only link tokens to the same vehicles but not PCs since they are provisioned by RSUs, and thus anonymity is preserved, as well.

\vskip3mm \noindent\textbf{Distributed \& Edge-Computing:} The main difference between DVSS and SCMS is that the DVSS, by design, inherits the advantages of the distributed and edge-computing paradigm since it relies on RSUs for the PC provisioning process and PCRL distribution. These advantages include:

\vskip3mm \noindent\textit{Fast Response Time:} In DVSS, the communication for PC provisioning between the vehicle and the RSU takes places at the link-layer of the network stack as a single Local Area Network roundtrip request whereas in the SCMS the PC request must travel through the entire network up to the SCMS backend system for a new PC to be provisioned. This is an important factor due to the high-speed nature of vehicles which results in short connection time; entering and exiting the RSU coverage within a short period. Our simulation in Section~\ref{sec:simulation}  demonstrated the inability of the SCMS to provide a new PC in a timely manner under the constraint of short vehicle-RSU connection time.

\vskip3mm \noindent\textit{Operates in Disconnected Environments:} Due to the edge-computing paradigm followed by DVSS, RSUs can provision new PCs even if the connection with the backend system is disrupted or lost, which is unlike SCMS where PCs are only provisioned via the backend system which requires stable network conditions.

\vskip3mm \noindent\textit{Distributed Computational Loads:} VPKI is inherently one of the largest PKIs in the worlds (350 million vehicles in the US, each with multiple PCs) and therefore a scalable system design such as DVSS is required where the computational loads of provisioning new PCs is distributed among RSUs, which is unlike the SCMS where the the load of provisioning new PCs for the whole country is concentrated in the backend system.
% Does the SCMS need a single-point-of-view to function or it can be divided into multiple backend systems, say, one for each state?

% Please note if tweaking SCMS so that it  completely delegates PC generation to RSUs  causes violation of unlinkability and anonymity in case of RSU compromises (\ie adversaries have easier access to RSUs);  our proposed system however is not prone to this threat.

% Note that the above commented information is moved to "Simple Architectural Design".

==> background_scms_old.tex <==
\section{Background}
\label{sec:background}

The Security Credential Management System (SCMS) was originally developed and published by \cite{Brecht2018SCMS} and adopted by the USDOT as the official vehicle's security framework for future applications of connected and autonomous vehicles \cite{USDOTSCMS}. As we will see in the related work in Section \ref{sec:related}, there is little exposure on the SCMS by the research community despite the fact that this system has been officially adopted by a government agency. Since our work in this paper will focus on the USDOT assumptions and requirements, in this section, we will provide a brief background on the original SCMS developed by \cite{Brecht2018SCMS}. Figure~\ref{fig:scms and dvss arch} shows an overview of the SCMS architecture. Readers who are not familiar with the cryptography used in this paper is urged to look at Appendix~\ref{sec:crypto prelim}.

 

% \begin{figure*}[h]
% % \vspace{-5pt}
% \centering 
% \includegraphics[width=.9\linewidth,keepaspectratio]{Images/SCMS overview 3.png}
% % \vspace{-6pt}
% \caption{SCMS Architecture Overview~\cite{CV2019USDOT}.}
% % \ahmed{Is this your diagram?} \abdulrahman{this diagram is brought from the SCMS conference paper}
% \label{fig:scms overview}
% % \vspace{-12pt}
% \end{figure*}

% \subsection{Main Functions}
\subsection{SCMS Overview}
In this subsection, we provide a high-level overview of the the main functions in SCMS. The details of each function is explained in detail in the next subsections.

\vskip3mm\noindent\textbf{Device Bootstrapping:} The main goal of the SCMS is distributing digital certificates to vehicles for secure and privacy-preserved communications among the vehicles themselves and between the vehicles and the SCMS backend system. The first step for any vehicle joining the system is obtaining a long-term certificate, called Enrollment Certificate (EC), signed by an Enrollment Certification Authority (ECA), as well as other important information such as public certificates of several SCMS authorities. A vehicle's EC acts as a passport that allows the vehicle to send authenticated service requests to the SCMS backend

\vskip3mm\noindent\textbf{Pseudonym Certificate Provisioning:} Once a vehicle owns an EC (which only happens once for each new vehicle or vehicle ownership transfer), the vehicle can request multiple Pseudonym Certificates (PC) and sign that request using its EC. The main purpose of PCs is to allow vehicles to communicate securely and anonymously among each other by swapping between PCs (e.g. every 5 minutes) in order to prevent an observer from tracking a vehicle by observing the same certificate signatures across two or more different locations. The current SCMS parameters allow a vehicle to have 20 to 40 PCs that are simultaneously valid for one week. All PC requests are sent to an SCMS entity called Registration Authority (RA) that validates, processes, and forwards requests for PCs to a Pseudonym Certification Authority (PCA). The PC provisioning process is described in details in Section \ref{sub:pc_provisioning}

\vskip3mm\noindent\textbf{Preserving Anonymity \& Unlinkability:}
From the PC provisioning process described above, one can see that the process of creating PCs is divided between two separate SCMS entities, RA and PCA. The main reason of this design is to prevent a single SCMS entity from linking the actual vehicle's identity (i.e. EC) to its corresponding PCs (\emph{anonymity}). In other words, the PCA cannot tell which of the PCs it has created belong to which vehicle since the requests are coming from the RA. Likewise, the RA cannot peek into the PCs (encrypted with the vehicle's public key) when it forwards the PCs to the vehicle. Furthermore, the RA shuffles the PC requests before sending it to the PCA to prevent the PCA from determining if two or more PCs belong to the same vehicle (\emph{unlinkability}). To preserve the vehicles' location anonymity, whenever a vehicle needs to communicate with the backend system, it communicates via an SCMS gateway called Location Obscurer Proxy (LOP) which has the role of obscuring the vehicle's location (i.e. IP address) by sending the vehicle's messages on its behalf to the desired SCMS destination server.



\vskip3mm\noindent\textbf{Misbehavior Reporting \& Certificate Revocation:} In case a vehicle is misbehaving (e.g. sending falsified information), other vehicles report this misbehavior to an SCMS entity called Misbehavior Authority (MA) and include the misbehaving vehicle's PC in the report. Once the misbehavior has been proven, the MA revokes all the currently active PCs of the vehicle by adding them in a Certificate Revocation List (CRL) to warn other vehicles from dealing with the culprit vehicle. The MA also adds the vehicle's corresponding EC in an internal EC Blacklist ($\BL$) that is only accessible by SCMS entities to prevent future PC requests from the blacklisted vehicle. The process of linking the PCs with its corresponding EC takes place among several entities and it is described in Section ~\ref{sub:scms_revocation}.


\subsection{Pseudonym Certificates Provisioning Process}
\label{sub:pc_provisioning}

When a vehicle wants to obtain a PC, it sends a PC request signed by its corresponding EC to the SCMS backend system via an RSU. First, the vehicle creates a PC public/private keypair $(g^x, x)$ and a session public/private keypair $(g^y, y)$. Then, the vehicle creates a PC request, attaches $g^x$ and $g^y$, signs it with its EC, then sends it to the backend system. The request is then relayed from the RSU to the RA via the LOP to hide the vehicle's location. Then for each PC request, the RA creates two sets of 20 random numbers \cut{$r_{i} \in $}$\{r_{1},\cdots, r_{20}\}$ and \cut{$r'_{j} \in $}$\{r'_{1},\cdots, r'_{20}\}$ (assuming the SCMS is configured to generate 20 PCs per request). The RA then raises $g^x$ to each $r_{i}$ and $g^y$ to each $r'_{i}$ for all ${i=1, \cdots, 20}$, creating 2 sets of 20 different public keys each, $\{g^{x.r_{i}}\}_i$ and $\{g^{y.r'_{i}}\}_i$; this process is known as Butterfly Key Expansion and its main purpose is to offload the creation of the 20 public keys to the RA (without knowledge of corresponding private keys) which reduces vehicle uplink bandwidth. After that, the RA sends each pair of ($g^{x.r_{i}}, g^{y.r'_{i}}$) to the PCA. Note that to preserve the unlinkability requirement, the RA shuffles between the pairs from different vehicles' requests before sending them to the PCA. This prevents the PCA from linking a group of keypairs (and ultimately PCs) to the same vehicle since PCA (according to the discrete log assumption) cannot distinguish if $g^{x.r_{i}},g^{x.r_{j}}$ are generated from the same PC request. The PCA then creates a random number $\hat r_{i}$ for each $g^{x.r_{i}}$ and raises it to that random number and signs the newly created PC public key using the PCA's private key, creating a PC$ = (g^{x.r_{i}.\hat r_{i}}, \sigma)$. The process of raising $g^{x.r_{i}}$ to a new random number $\hat r_{i}$ by the PCA is done to prevent the RA from linking multiple PCs to the same vehicle (preserving unlinkability) since the RA is the SCMS entity who performed the Butterfly Key Expansion process. It also prevents the RA from linking a PC to its corresponding EC (preserving anonymity) since it knows who is the requesting vehicle. After that, the PCA encrypts $\ct = $(PC, $\hat r_{i}$) using its paired $g^{y.r'_{i}}$ (which is received from the RA) and sends it back to the RA. Finally, the RA sends the newly signed PCs to the requesting vehicle by relying  $\{\ct, r_{i}, r'_{i}\}$ over a secure channel (\eg TLS). Note that the PCA and RA keep a \emph{request reference number} for each keypair in order for the RA to know which signed PC to send to which vehicle without the need of looking into the encrypted content of $\ct$. Upon receiving the response from the RA, the vehicle computes the expanded private key of each $g^{y.r'_{i}}$ as $y.r'_{i}$ and decrypt the PCA messages. It then computes the expanded private keys of each PC, $g^{x.r_{i}.\hat r_{i}}$ as $x.r_{i}.\hat r_{i}$.

\subsection{Enrollment \& Pseudonym Certificate Revocation Process}
\label{sub:scms_revocation}

\vskip3mm \noindent\textbf{Creating Linkability:} If a vehicle misbehaves, the SCMS should be able to link the vehicle's PC to its EC for revocation and accountability. 
% The PC provisioning process described in the previous section provides complete unlinkability even if all SCMS entities cooperate together (which is undesirable).
Naively, all non-expired PCs of a single revoked vehicle are added to the pseudonym certificate revocation list (PCRL) upon revocation; however, the PCRL size becomes extremely large and bandwidth consuming since SCMS generates a large number of PCs per vehicle. In order to have a fixed number of entries (namely one entry) required to be added in the PCRL per revoked vehicle regardless of the number of revoked PCs, SCMS links all PCs of  a single vehicle in such a way that no single entity in the system is able to distinguish their relation (and thus acheive unlinkability). To provide linkability of misbehaving vehicles, a Linkage Value $LV$ (\ie a PC id) is added to each $PC$ created by the PCA.

To create the $LV$, two SCMS entities are responsible for this task, called Linkage Authority 1 ($LA_{1}$) and Linkage Authority 2 ($LA_{2}$). For each newly created $EC$, each $LA$ creates and assigns a random number for that $EC$ called Linkage Seed 0 ($LS_{0}$) which will be used to create a hash chain of Linkage Seeds $LS_{i}$ such that $LS_{i+1} = H(LS_{i})$. Each $LS_{i}$ acts as a reference value for a batch of 20 $PCs$. The $LS_{i}$ is then used to create 20 different values called Prelinkage Values $PV_{j} \in (PV_{1},...,PV_{20})$ using an AES function such as $PV_{j} = \enc_{LS_{i}} (j||LA_{ID})$ where $LA_{ID}$ is the ID of the $LA$ which is used to prevent the chance of having the two $LAs$ randomly choose the same $LS_{0}$ seed for the same vehicle. Finally, each $PV_{j}$ from $LA_{1}$ and $LA_{2}$ for a given batch $LS_{i}$ are XORed together creating $LV_{i,j}$ ($LV$ for PC $j$ from batch number $i$). Notice that the creation of a single $LV$ is divided between two $LAs$ to prevent a single LA from linking multiple $PCs$ by simply looking at their $LVs$. Also, the PCA cannot retrieve  the two corresponding $LS_i$ given the two $PV_j$ only because it does not know the AES key (\ie $LS_i$). Furthermore, the XORing operation of the two $PV_{j}$ is done by the $PCA$ during the $PC$ creation process. Note that since the PCA does not know the EC of the requesting vehicle, the LAs cannot determine from which $LS_{0}$ seed the $PV$ should be derived from since the PCA cannot provide the EC to them. Therefore, the $PV$ request is done by the RA during the key expansion process (since it is the entity who knows the EC of the requesting vehicle and the batch number $i$) and passes it to the PCA. Furthermore, to prevent the RA from linking PCs to the same vehicle via their $LVs$ (by XORing its $PVs$), LAs encrypt the $PVs$ with the PCA's public key before passing them to the RA.

\vskip3mm \noindent\textbf{Revoking a Misbehaving Vehicle's Certificate:} Once a vehicle is determined to be misbehaving, the MA contacts the PCA and requests the 'PC request reference number' between the PCA and the RA that was used to create the misbehaving PC. Based on reference number, the MA instructs the RA to add the EC of the vehicle who requested the PC, to an SCMS internal blacklist (\BL) in order to prevent future PC provisioning requests from the misbehaving vehicle. Then the MA (with the help of RA) instructs the two LAs to reveal their $LS_{i}$ for the blacklisted EC (via EC initial seed $LS_{0}$) for a given batch $i$. Assuming the SCMS is configured to allow a vehicle to have 20 $PCs$ every week, each $LS_{i}$ represents the linkage seed of week $i$ for a vehicle. In other words, based on the validity time of a given PC, the batch number is inferred from the week number. After that, the two LAs add the $LS_{i}$ of the misbehaving vehicle to a public PCRL. Once the two $LS_{i}$ are made public, any vehicle can compute all subsequent $LS_{i+1}$, derive the $PV$ for week $i$, and XOR the $LVs$ of the misbehaving vehicle for all subsequent weeks until the vehicle's EC expiration date (or simply until the end of the current week since the misbehaving vehicle is blacklisted from any future PCs).

\subsection{Comparative Analysis Between DVSS \& SCMS}

\vskip3mm \noindent\textbf{Simple Architectural Design:} The design of the DVSS is far simpler than of the SCMS's which makes our system easier to maintain and extend with additional functionalities without risking a cascade of changes across other system's components. As discussed in section \ref{sec:background}, the SCMS requires multiple entities with complex relationships among them to preserve the anonymity and unlinkability of vehicles. On the other hand, DVSS enables vehicles to acquire PCs in two simple phases, tokens acquisition phase, $\tokengen$, (a vehicle requests a set of tokens from the DVSS backend system before the start of the trip such as when the vehicle is parked at night), and PC provisioning phase, $\pseudogen$, (a vehicle provides an RSU with a token in exchange for a new PC). Importantly, each phase requires communication with a single system entity.  With this simple -yet effective- design, the anonymity, unlinkability, and revocability of vehicles are preserved without complex interactions between system entities. For instance, if the SCMS decided to push the PC provisioning to the RSUs, this would put the RSUs (and ultimately the anonymity and unlinkability of vehicles) at risk since RSUs are physically accessible to malicious parties and any compromised RSU would potentially compromise the security of the system. In DVSS, compromised RSUs won't reveal any identifying information to the attacker since the tokens received by the RSUs are anonymous by design.

\vskip3mm \noindent\textbf{No Sybil Attack:} The SCMS allows a vehicle to hold onto multiple PCs that are simultaneously valid at the same time. This enables a misbehaving vehicle to launch what is known as Sybil Attack where the misbehaving vehicle communicates with other vehicles/RSU with multiple identities. This attack could -for example- give the impression of a congested road or intersection which might influence the behavior of other vehicles/RSUs such as a smart intersection controller extending the green light of the congested intersection lane. On the other hand, a vehicle under the DVSS can hold onto multiple tokens, each with a non-overlapping validity period. In other words, a vehicle can request multiple PCs with multiple tokens but each PC will have a validity period that is different from the rest of the PCs. If a misbehaving vehicle tries to request multiple PCs from different RSUs simultaneously, each PC can only be used in a unique region, which makes Sybil attacks unfeasible; this particular case however causes clone attacks, which our system handles as will be shown later.

\vskip3mm \noindent\textbf{Short PCRLs:} As discussed in Section~\ref{sec:intro}, the size of a PCRL in SCMS is $N\times |V'|$ where $N$ is the number of active PCs per vehicle and $|V'|$ is the number of revoked vehicles. If we assume 1\% of the US vehicles are revoked, and the SCMS allows a vehicle to have 20 simultaneously active PCs, then the number of entries in the PCRL that each vehicle must maintain is 70 millions which is not very scalable for a vehicular network; likewise, the PCRL requires high bandwidth because of its large size even after utilization of the hash chain mechanism (\ie PCRL would have 3,500,000 entries). A possible solution is confining the validity of PCs within a predefined geographical area where each area has its own PCRL. However, adding a validity-location attribute to a PC would violate the unlinkability of vehicles
% , either by RA or PCA
by PCA or anonymity by RA
(depending on the design choice of who the location handler is). Another mitigating approach (which is suggested by the SCMS) is dividing the PCRL into multiple PCRLs based on some attribute such as the region of misbehavior. However, since a vehicle could have a week-worth of PCs, a misbehaving vehicle might travel outside the regional PCRL and remain unrevoked in neighboring regions. In DVSS, each RSU is responsible for providing PCs within its region. Therefore, it is possible for an RSU to issue a PC that is confined within its region of control without violating the unlinkability of vehicles since the linkability information is embedded with the tokens (which is provided by the DVSS CA), not the PCs. In other words, the CA can only link tokens to the same vehicles but not PCs since they are provisioned by RSUs, and thus  anonymity is preserved, as well.

\vskip3mm \noindent\textbf{Distributed \& Edge-Computing:} The main difference between DVSS and SCMS is that the DVSS, by design, inherits the advantages of the distributed and edge-computing paradigm since it relies on RSUs for the PC provisioning process and PCRL distribution. These advantages include:

\vskip3mm \noindent\textit{Fast Response Time:} In DVSS, the communication for PC provisioning between the vehicle and the RSU takes places at the link-layer only as a single Local Area Network roundtrip request whereas in the SCMS the PC request must travel through the entire network up to the SCMS backend system for a new PC to be provisioned. This is an important factor due to the high-speed nature of vehicles which results in short connection time; entering and exiting the RSU coverage within a short period. Our simulation in Section~\ref{sec:simulation}  demonstrated the inability of the SCMS to provide a new PC in a timely manner under the constraint of short vehicle-RSU connection time.

\vskip3mm \noindent\textit{Operates in Disconnected Environments:} Due to the edge-computing paradigm followed by DVSS, RSUs can provision new PCs even if the connection with the backend system is disrupted or lost, unlike SCMS where PCs are only provisioned via the backend system which requires stable network conditions.

\vskip3mm \noindent\textit{Distributed Computational Loads:} VPKI is inherently one of the largest PKIs in the worlds (350 million vehicles in the US, each with multiple PCs) and therefore a scalable system design such as DVSS is required where the computational load of provisioning new PCs is distributed among RSUs, which is unlike the SCMS where the the load of provisioning new PCs for the whole country is concentrated in the backend system.
% Does the SCMS need a single-point-of-view to function or it can be divided into multiple backend systems, say, one for each state?

% Please note if tweaking SCMS so that it  completely delegates PC generation to RSUs  causes violation of unlinkability and anonymity in case of RSU compromises (\ie adversaries have easier access to RSUs);  our proposed system however is not prone to this threat.

% Note the above commented information is moved to "Simple Architectural Design".

==> design_overview.tex <==
\section{System Overview}
The system consists of the following players: a set of vehicles $\V=\{v\}$, a set of road-side units $\RSU=\{\rsu\}$, and a certificate authority $\CA$.  The goal of the system is to provide the vehicles with temporary, anonymous, authenticated certificates $-$ \emph{pseudonym certificates} $-$ which they will use to authenticate their communications as they drive around.  The pseudonym certificates are assigned (and revoked) in four stages, corresponding to the four subroutines $(\setup,\tokengen,\pseudogen,\revoke)$ which govern how the players interact with one another.  In order to demonstrate how these protocols fit together to comprise the scheme, let us follow a vehicle $v\in V$ as it navigates its way through the system.

To begin, $v$ and $\CA$ run $\setup$, by which $v$ obtains an authenticated ``long term certificate'' $\ltc_v$ which will not change.  $\setup$ is run once, ideally by the vehicle manufacturer.  Next, but still prior to $v$ entering the network, $v$ and $\CA$ run $\tokengen$ which grants $v$ a set of tokens $\T=\{\tau_1,\dots,\tau_N\}$.  This is an authenticated interaction, meaning that $\CA$ will not grant the tokens to $v$ unless $v$ authenticates itself using $\ltc_v$.  The $i-$th token, $\tau_i$ will be valid only during the $i-$th period of time; when the $N-$th time period ends, $v$ will have to run $\tokengen$ again to get more tokens.

Once $v$ has obtained tokens, it can begin driving, though it cannot yet communicate with other vehicles.  When it encounters its first roadside unit, $\rsu\in\RSU$, $v$ and $\rsu$ execute $\pseudogen$ which grants $v$ a pseudonym certificate PC for a specific time period.  This is also an authenticated interaction; $v$ must use its token $\tau$ corresponding to the current time period in order to get a valid PC.  When the time period expires, $v$ will have to run $\pseudogen$ again with another $\rsu'\in\RSU$ using its next token in order to get a new PC.  Armed with a pseudonym certificate, $v$ is now able to securely communicate with other vehicles as it drives around.  If $v$ misbehaves (\emph{e.g.}, maybe $v$ broadcasts bogus traffic information in order to encourage cars to avoid the highway so to give itself a faster commute), $v$ risks being revoked from the system.  In case $v$'s bad behavior is noticed by $\rsu$, $\rsu$ and $\CA$ will execute the $\revoke$ subroutine.  Roughly speaking, $\rsu$ alerts $\CA$ that a certain token $\tau$ belongs to an adversarial vehicle.  $\CA$ will connect $\tau$ to the vehicle $v$ and broadcast all of $v$'s tokens to all nearby roadside units, thus preventing $v$ from being able to obtain any other pseudonym certificates (after its current one expires).  Notice that since each token is valid only for a specific time period, the list of revoked tokens does not need to include old expired tokens, so it can remain small.

\vskip 3mm\noindent{\bf Cryptography Under the Hood.} The above discussion mentions authenticated interaction and certificates, which are implemented using digital signatures.  For example, during the $\setup$ subroutine, $v$ draws a signature key pair $(\vk_v,\sk_v)$, and send $\vk_v$ to $\CA$.  $\CA$ uses its own signature key pair $(\vk_\CA,\sk_\CA)$ to sign $\vk_v$, obtaining $\sigma_v=\sign_{\sk_\CA}(\vk_v)$, which it returns to $v$.  The signature $\sigma_v$ can be verified by anyone in the system (since $\vk_\CA$ is public).  The long term certificate $\ltc_v$ is the pair $(\vk_v,\sigma_v)$, and $v$ can authenticate itself to other users in the system by signing messages using $\sk_v$.  These details appear in the formal presentation of the system in the next section.





\subsection{System Security} In order to ensure the privacy of the vehicles as they move through the system, two additional security features $-$ \emph{anonymity} and \emph{unlinkability} $-$ are required.  We also discuss \emph{sybil attacks} and \emph{clone attacks}.

%\vskip 3mm
\noindent{\bf Anonymity.} This requires that the roadside units do not learn the true identities (\emph{i.e.}, the long term certificates) of the vehicles.  Intuitively, this is achieved in our system because the tokens do not reveal any information about the long term certificate used during $\tokengen$ to obtain them.

%\vskip 3mm
\noindent{\bf Unlinkability.} This requires that $\CA$ cannot trace the vehicle pseudonyms back to the long term certificates, even if they can observe the communications on the road.  This is achieved in our system because the pseudonym certificates do not reveal any information about the tokens used to obtain them during $\pseudogen$.  The mechanism for security here is identical to the one for anonymity.

%\vskip 3mm
\noindent{\bf Sybil Attacks.} This requires that $v$ have multiple pseudonyms that would allow it to authenticate messages under different identities at the same time and region. These are prevented because each token can be redeemed one time within a specific time period and region during $\pseudogen$.
% \silas{Explain what these are and why they're not an issue for us...}

%\vskip 3mm
\noindent{\bf Clone Attacks.} This requires that $v$ have multiple pseudonyms that are valid at the same time but different regions. These attacks are mitigated in our system by reporting consumed tokens to a single database and revoking the corresponding $v$.
% \silas{Need a new name?  Also, explain what these are how we stop them...}

% \vskip 3mm\noindent{\bf Threat Model.}  We assume the backend servers are trusted but curios parties. We also assume that RSUs are easier to compromise since they are more accessible to adversaries; they are also curious and might collude with one another in an attempt to launch any of the aforementioned attacks. We assume the $\CA$ and an RSU do not collude. We do not consider  denial of service (DoS), jamming and Radio Frequency (RF) fingerprinting~\cite{brik2008wireless} attacks.


\subsection{System Improvements}
% We here describe the benefits that vehicles get when using our system.
We here describe  the system improvements from the viewpoint of vehicles.



\vskip 3mm\noindent{\bf Low Latency PC Generation.}
A vehicle $v$ is always able to get a new PC while driving fast (and being disconnected from the backend). This is achieved because $\pseudogen$  requires  a single-hop communication with  $\rsu$. $\rsu$ can locally verify a token $\tau$ since it is signed by $\rsu$'s authority (\ie $\CA$); $\rsu$ can locally sign a new PC because it has a signing certificate.


\vskip 3mm\noindent{\bf Spatiotemporal PCRL.}
$v$ is always able to download pseudonym certificate revocation lists (PCRL) during its short-time connectivity with $\rsu$. This is achieved because each PCRL is only valid for a single area and a short-time interval, which significantly reduces the PCRL size (and thus the bandwidth requirements).


\vskip 3mm\noindent{\bf Quick Revocation.}
Our system shortly eliminates revoked vehicles from participating in VANET even in worst cases where a PCRL is not downloaded by $v$.
% A revoked vehicle $v'$ only has short time to misbehave after $\revoke$ is executed (\ie till the end of current time period).
This is because  $\pseudogen$ must periodically be executed, which  outputs a new PC only if a presented $\tau$ is not revoked.



\vskip 3mm\noindent{\bf Scalability.}
$v$ is always able to get a new PC regardless of the number of vehicles in the system. This is achieved in our system because $\pseudogen$ workload is distributed on the infrastructure;  $v$ always executes $\pseudogen$ with a nearby $\rsu$.


% \vskip 3mm\noindent{\bf PC Generation under Stringent Network Conditions.}
% $v$ is always able to get a new PC. This is achieved because PC generation only requires a single-hop communication with $\rsu$ and does not require online participation from the backend.

% $\rsu$ can locally verify a token $\tau$ since it is signed by $\rsu$'s authority (\ie $\CA$); $\rsu$ can locally sign a new PC because it has a signing certificate.



% \vskip 3mm\noindent{\bf No CRL.}
% A vehicle $v$ does not download and maintain a CRL to detect a revoked vehicle $v'$. This is because $v'$ only keeps tokens for future time periods, which cannot be used to authenticate messages; thus, only \emph{road-side units} need to download and maintain a token revocation list ($\TRL$).

% once $\revoke$ is executed to revoke $v'$, $\pseudogen$ run between $v'$ and $\rsu$ does not output a $\psc'$. $\pseudogen$ must be executed periodically.




% $\pseudogen$ to be able to continue authenticating messages; $\pseudogen$ outputs a new $\psc$ only if $\tau$ is not revoked.


% , which has a signing certificate.

% This is achieved in our system because $v$ executes $\pseudogen$ with a nearby $\rsu$; thus, $\pseudogen$ workload is distributed.

% $\pseudogen$ is being performed by the infrastructure $\rsu$. 


% \vskip 3mm\noindent{\bf No CRL.}
% An essential feature of our system is the ability to protect legitimate vehicles from malicious vehicles while relieving legitimate vehicles from having to frequently download and store \emph{large} CRLs. Our system, unlike other schemes, achieves this feature because it does not allow a vehicle $v$ to keep future pseudonym certificates (\ie it rather keeps a token list $\T$, which cannot be used for signing messages).
% This allows legitimate vehicles in our system to be assured that a compromised vehicle $v'$ will soon be unable to participate in the system since its pseudonym certificate  expires soon, and the infrastructure  will not grant $v'$ a new pseudonym; thus, no need for legitimate vehicles to download a CRL.  This is an important feature because CRL size becomes highly bandwidth-consuming overtime and hard to download, especially in vehicular environments where vehicles only get short-time network connectivity. Our system eliminates this responsibility from vehicles and rather assigns this responsibility of keeping a revocation list (\ie token revocation list $\TRL$) to the infrastructure, which does not have this network connectivity limitation. 

% In order to avoid having a large token revocation list $\TRL$, we additionally introduce a mechanism that allows the $\CA$ to publish a trapdoor that enables $\rsu$ to link tokens of a single vehicle such that only one value (\ie token $\tau$) per revoked vehicle $v'$ needs to be published in the $\TRL$; this makes the space complexity of $\TRL$ be $\mathcal{O}(|\V|)$ rather than $\mathcal{O}(\mathcal{|T|})$, where $\mathcal{T}$ represents the set of all tokens in the whole system (\ie $\T\subset\mathcal{T}$). This presents a significant reduction in the size of $\TRL$. This mechanism is flexible so that it can allow the $\CA$ to publish a trapdoor that allows $\rsu$ to link only portion of the token list $\T'\subset\T$ of $v'$ (\eg only  revoked tokens) while ensuring unlinkability of the $v'$ other tokens $\T''\subset\T,$ where $\T'\cap\T'' = \emptyset$ ; This allows our system to also guarantee unlinkability of tokens (or pseudonyms) of the revoked vehicles before they were revoked (\ie retrospective unlinkability).



% \vskip 3mm\noindent{\bf Quick Revocation.}
% Our system guarantees that revoked vehicles are shortly eliminated from participation in the system, which increases the overall security of the system (and thus safety and efficiency of connected vehicles). It utilizes the fact that $v$ needs to periodically switch to a new a pseudonym by implicitly making this process a chance for the infrastructure to check $v$'s revocation status (\ie checking if $\tau$ is not revoked) before generating a new short-lived pseudonym to $v$.  This allows other vehicles to believe that $v$ with a non-expired pseudonym is likely not revoked. The advantages of this approach are 1) this process does not require extra bandwidth specific for the revocation status information, and 2) all vehicles are constantly required to follow this process in order to get a new pseudonym certificate and participate in the system. 


% \vskip 3mm\noindent{\bf Low Latency.}
% Our system realizes the fast mobility of connected vehicles along with the too time-limited network connectivity that they get while driving. Since network latency is the bottleneck in vehicular communication environments, frequent reliance on a distantly faraway cloud $\CA$ becomes unreasonable as vehicles soon lose network connectivity, which leads to protocol failure. Therefore, our system moves the whole pseudonym certificate renewal operations at the edge closer to the vehicles and allows the recipient $\rsu$ to both anonymously verify $v$ using a temporary token $\tau_i$ and create the new pseudonym to $v$ without the need for any extra communications. $\tau_i$ carries a uniquely random $\id$, that can only be used by the $\CA$ to trace $v$ if needed, and a signature $\sigma$ by the $\CA$ that tells $\rsu$ to accept $v$ as a legitimate anonymous $v$ during the $i-$th time period.    This allows our system to significantly expedite pseudonym certificate generation as it only needs a single round trip time (RTT) between two nodes (\ie $v$ and $\rsu$) that are in a physically close area.  This also allows our system to work under stringent situations, where connectivity between $\rsu$ and the $\CA$ is intermittent and unstable, such as $\rsu$ in rural areas relying on wireless internet service providers, satellite communication ..etc.


% \vskip 3mm\noindent{\bf Scalability.}
% The large size of users and the privacy requirements in vehicular communication systems  impose huge computational burden on the cloud (\ie $\CA$). Such a system is constantly growing, as it is expected to also serve pedestrians, cyclists, trains, drones ...etc. This places huge costs on the $\CA$ as it needs to keep investing in its resources to allow the system to scale. Our system takes advantage of the compute power in the already existing $\RSU$ by distributing computation overhead of issuing new pseudonym certificates on $\rsu\in\RSU$. This is achieved by letting our key management system become hierarchical, where the $\CA$ delegates the pseudonym certificate generation privilege to $\rsu$ by providing them certificates that allow signing pseudonym certificates for vehicles.    This allows our system to utilize the infrastructure to help it scale without the system incurring extra costs.


\vskip 40mm
















==> old_intro.tex <==

Furthermore, connectivity with the outside network is scarce in CV environments as vehicles often rely on the infrastructure (aka road-side units, $\RSU$) to connect with the $\CA$; thus, it becomes infeasible for vehicles to refresh their pseudonyms while they drive around. Vehicles need to wait for the $\CA$ response with fresh pseudonym certificates before they are out of network coverage of $\rsu\in\RSU$; however, considering the nature of vehicles often moving at high speeds (\eg on a highway), this approach becomes impractical due to high network latency. In many cases, connectivity between $\rsu$ and $\CA$ can additionally be intermittent, which increases total network latency and results in vehicles failing to refresh pseudonyms and anonymously participate in the VANET.  Thus, VPKI must be able to issue pseudonyms at low network latency to be practical. 

Previous work on VPKI (\eg~\cite{Brecht2018SCMS}) tries to avoid the need for vehicles to have frequent connectivity with the $\CA$ by pre-loading them with a batch of pseudonyms that allow them to anonymously authenticate messages for long time periods (\eg a year worth of pseudonym certificates).  This choice  however introduces two issues: 1) a revoked vehicle $v'$ can continue authenticating messages till the last pseudonym certificate expires (\eg till the end of the year) as long as other vehicles are not notified of $v'$ misbehavior, and 2) the certificate revocation list (CRL) size significantly increases as it now needs to include all revoked pseudonym certificates of $v'$. Therefore, there is an inverse relationship between availability of network connectivity with the pseudonym certificate issuer (\ie $\CA$) and the CRL size.





\begin{table*}[]
    \centering
        
    \scalebox{.85}{
    \begin{tabular}{l|c|c|c|c|c}
        CA & Number of Unique CRLs & Minimum CRL size (KB) & Average CRL size (MB) & Maximum CRL size (MB) & Total CRL size (MB) \\
        \hline
        Apple & 28 & 0.29 & 7 & 196.4 & 198.6 \\
        Cloudflare & 1 & 21,380.28 & 20.8 & 20.8 & 20.8 \\
        Actalis & 2 & 49.3 & 9.3 &   18.5 & 18.5\\
        Google  & 3 & 4.53 & 5.2 & 15.5 & 15.7 \\
        Digicert & 46 & 0.29 & 0.8 & 15.4 & 38.8\\
        Entrust & 2 & 247.32 & 1.5 & 2.8 & 3.1 \\
        Sectigo & 11 & 0.51 & 0.2 & 1 & 3 \\
        GoDaddy & 750 & 18.43 & 0.1 & 1 &  74.5 \\
    \end{tabular}
    }
    \vspace{6pt}
    \caption{Certificate revocation lists (CRLs) statistics for major certificate authorities (CAs) in the internet.}
    \label{tab:crl stats}
    
\end{table*}

To get a sense of a potential CRL size in VPKI, one could consider the regular revocation percentage in another similar domain, namely the internet, which is $\sim1.29\%$~\cite{smith2020let}; considering the US scenario with 350 million vehicles, this would result in a VPKI CRL with at least 4,515,000 certificates (\ie 177 MB). Moreover, we collect and show CRL statistics of major $\CA$s in Table~\ref{tab:crl stats} to show how large actual CRLs can be (as of November 2020). Downloading the CRL becomes a significant issue, especially in environments where network bandwidth is limited, such as the vehicular environment. As a result, vehicles would end up becoming unaware of revoked malicious vehicles. 
There are proposals to divide the CRL into multiple pieces in order to allow vehicles to download individual CRL pieces at different time points; for example, such pieces can contain increments as new revocations are reported.  This type of solutions however does not solve the issue since the rate of revocations is not expected. For instance, consider the cyber attack in 2015 which allowed hackers to disable vehicles; this attack triggered Chrysler to recall 1.4 million vehicles~\cite{Cyberhac5:online}. Thus, the CRL (or all its pieces) is useful if it can  always be fully downloaded by vehicles. Coupled with the fact that network connectivity is intermittent in vehicular environments, this introduces a concern on how long time is needed till all revoked vehicles are detected by other vehicles.

We propose a novel  key management system that improves security, efficiency and scalability in vehicular environments.
At the heart of our solution, we utilize deployed infrastructure ($\RSU$) by letting it completely handle  key management recurring operations that are traditionally handled by the $\CA$. This is not trivial in vehicular environments since vehicles demand being able to request pseudonym certificates without being identified or linked by the system.  Our system achieves these demands by leveraging pre-generated anonymous tokens that allow a vehicle to anonymously redeem them for pseudonym certificates.  Thus, the proposed key management system is able to provide major advantages over previous systems as shown next.

\vskip 3mm\noindent{\bf No CRL.}
An essential feature of our system is the ability to protect legitimate vehicles from malicious vehicles while relieving the former from having to frequently download and store \emph{large} CRLs.  This is an important feature because CRL size becomes bandwidth-consuming overtime and hard to download, especially in vehicular environments.

\vskip 3mm\noindent{\bf Quick Revocation.}
Our system shortly eliminates revoked vehicles from participating in VANET. This increases the overall security of the system, and thus safety and efficiency of connected vehicles.

\vskip 3mm\noindent{\bf Low Latency.}
Our system lowers the network latency needed for a vehicle to refresh its pseudonym certificate. This is important for vehicles as they only have intermittent connectivity. 

\vskip 3mm\noindent{\bf Scalability.}
Our system leverages the infrastructure to issue pseudonyms, which helps it organically scale. This is important because the vehicular environment is such a large scale system that could impose significant costs if not designed carefully.



==> old_sys_overview.tex <==

% The reason they are anonymous and temporary is because we need to stop curious entities (e.g., vehicles, RSUs or even the backend system) from using vehicle's messages to track its long-term driving activities. In other words, the system needs to achieve the anonymity and long-term unlinkability properties, which become a challenge when designing such a system. Anonymity ensures that a vehicle real identity is not revealed as a result of its authenticated vehicle to vehicle (V2V) communications. Long-term unlinkability ensures that pseudonym certificates of a single vehicle used in V2V communications cannot be linked to the same vehicle. 
In a vehicular communication environment,  the assumption is that road-side units (RSUs) are always deployed across roads and highways, and connectivity with the backend is only available through them.  Because RSUs have a small network coverage area and might have intermittent connectivity with the backend (\eg consider a rural area where RSUs rely on wireless internet service providers, WISPs), vehicles often have short-time connectivity with RSUs (e.g., consider a vehicle driving on a highway) and have no frequent stable connectivity with the backend.
% To fix this issue, our system provides the infrastructure with the ability to instantly refresh pseudonym certificates for vehicles while still achieving anonymity and long-term unlinkability.

In our system, we assume the backend and RSUs are equipped with pairs of asymmetric encryption and decryption keys, $(\ek_\B,\dk_\B)$ and $(\ek_{RSU},\dk_{RSU})$ respectively. Also, the backend has a pair of asymmetric signing and verification keys $(\sk_\B,\vk_\B)$ and a self-signed certificate $\ltc_\B$ that is the root of trust in the system; this backend could be the Department of Motor Vehicles (DMV), Department of Transportation (DoT) ..etc. Each RSU has a pair of $(\sk_{RSU},\vk_{RSU})$ and a certificate $\ltc_{RSU}$ signed by the backend; this certificate allows an RSU to generate pseudonym certificates for vehicles. Each manufacturer also has a pair of $(\sk_{m},\vk_{m})$ and a certificate $\ltc_m$ signed by the backend; this certificate is used for attesting vehicle requests to get long-term certificates.  Communications between vehicles, RSUs and the backend always occur over a secure channel (\eg TLS). We also assume that all communications with the backend pass through a location obscurer proxy that conceals network addresses in order to hide the other party's physical location from the backend. 



\subsection{Notations}
We here set some notations.  $x\leftarrow\$$ means $x$ is assigned a random value. $(\ek,\dk)$ denote a pair of asymmetric encryption and decryption keys, respectively. $(\sk,\vk)$ denote a pair of asymmetric signing and verification keys, respectively. $\ltc$, $\pc$ and $\ac$ denote long-term and pseudonym certificates, respectively, where $\{\ltc, \pc\}\leftarrow(\vk, \sigma)$ for $\sigma$ is a signature on $\vk$. $\st,\et$ denote  start and end times of a time window $\tw$, respectively. $\TF=\{\tw_1, \cdots, \tw_N\}$ denotes a list of unique time windows, where $\tw_{i+1}>\tw_i$.  $\T = \{t_1, \cdots, t_N\}$ denotes a list of tokens, where tokens $t_i,t_{i+1}\in\T$ are valid at time windows $\tw_i,\tw_{i+1}$, respectively. A token contains $t\leftarrow(\id, \tw, \sigma)$, where $\id$ is a token identity, and token's content $\tc\leftarrow(\id, \tw)$.   $\BL$ denotes a long-term certificate black list, which is local to the backend $\B$. $\TRL$ denotes a token revocation list, which is updated by the backend and distributed to RSUs. $\UTL$ denotes a local list of tokens that has been seen by an RSU. $\pt, \ct, \msg$ denote a plaintext, ciphertext and message, respectively. 

\subsection{System Model and Assumptions}




\subsection{System Overview}
Our system consists of four algorithms (\setup, \tokengen, \pseudogen, \revoke). Roughly speaking, $\setup$ is only run once per vehicle to produce a long-term certificate. $\tokengen$ is run whenever a vehicle needs to get a list of authorization tokens (e.g., once a week, month, year ..etc) that allow it to request short-term pseudonym certificates. $\pseudogen$ is run whenever the vehicle needs to get a short-term pseudonym certificate that allows it to communicate anonymously with other vehicles.  $\revoke$ is invoked to revoke the privileges of a misbehaving vehicle to prevent it from participating in the system.  We begin with a high level discussion of each algorithm.


Our system consists of four algorithms (\setup, \tokengen, \pseudogen, \revoke). When a vehicle is about to be  used for the first time, it needs to go through a setup protocol $(\setup)$ to get a long-term certified identity (\ie long-term certificate); such certificates are the means that allows legitimate vehicles to authenticate themselves when communicating with the backend system. In order to improve passenger safety and road efficiency in a vehicular environment, vehicles are urged to share their road observations with nearby vehicles to allow for better driving decisions;   such observations need to be shared in an authenticated manner to prevent adversaries from degrading road efficiency or causing road accidents. Naively, a vehicle would authenticate such observations using its long term certificate and broadcast them to other vehicles. However, this proposes privacy concerns as the vehicle's messages carry its real identity; this could allow the backend, RSUs, manufacturers or other vehicles to collect such messages and track the vehicle's driving activities. Therefore, a vehicular communication system needs to anonymize vehicle identities; \emph{anonymity} ensures that a vehicle real identity is not revealed (to the backend, RSUs, manufacturers and other vehicles) as a result of its authenticated vehicle to vehicle (V2V) communications. While the backend could additionally, at $\setup$, provide a pseudonym identity for anonymous V2V communications,  it still can identify  messages of a single vehicle since the backend knows the corresponding long term and pseudonym identities  (\ie no anonymity from the backend). One way to overcome this issue is to divide this process into two tasks and assign them to two nodes within the system (\ie two nodes at the backend), where one does long-term certificate verification and the other creates pseudonym certificates; 
% this solution introduces other issues as will be discussed below.

While anonymity conceals a vehicle's identity, it still does not conceal its driving activities; this provides valuable information for eavesdroppers that allows  route tracking (which might eventually be linked to the vehicle, say if a vehicle is compromised). One way to address this issue is to allow the vehicles to have multiple pseudonym identities (\eg multiple pseudonym certificates, group signature schemes ..etc); however, it is important to note that this same approach could allow for masquerading as multiple vehicles (\ie a Sybil attack) if multiple pseudonym identities could be used at the same time window. One seemingly proper way to utilize this approach is to make vehicles use a pseudonym certificate for a single message communication only; while this approach achieves optimal unlinkability, this is not desirable in vehicular environments.  Linking messages of a single anonymous vehicle for a period of time (\eg several minutes) is important as it enables other vehicles to make critical driving decisions; for example, it helps connected vehicles to use broadcast messages of other vehicles to avoid crashes as a result of unexpected behavior of other surrounding vehicles (\eg critical connected vehicle applications: forward collision warning FCW, Emergency Electronic Brake Light EEBL ...etc).      Therefore, a vehicular communication system only needs to hide the \emph{long-term} driving activities of a single vehicle in order to prevent tracking; \emph{long-term unlinkability} ensures that pseudonym certificates of a single vehicle used in V2V communications cannot be linked to the same vehicle. One way to achieve this property is to pre-load a vehicle with a set of consecutively valid independent pseudonym certificates (\eg a year worth of certificates). However, in case of a vehicle compromise, the attacker is able to participate in the system till the end of the year; certificate revocation lists (CRLs) can be used to mitigate this attack, but they grow large over time and it becomes too large to download them especially for vehicles with short-time network connectivity. Another solution is to make vehicles periodically refresh their pseudonym certificates whenever they get connectivity (\ie be in an RSU vicinity), but this is not reasonable in vehicular environments due to intermittent connectivity and long network latency with the backend.

In order to design a system that avoids all the aformentioined issues, our system delegates the pseudonym certificate generation task completely to the infrastructure. A vehicle runs a token generation protocol ($\tokengen$) which allows it to get a list of tokens $\T = \{t_1,\cdots,t_N\}$; each token $t_i$ serves as an authorization from the backend that the vehicle can use to refresh a pseudonym certificate at time window $\tw_i$. Note that this is the only process that requires the vehicle to communicate with the backend system, and it takes place only one time for some time period (\eg once a year). Most importantly, tokens have no values that can be used to reveal vehicles' identities. This limits the attacker ability when compromising a vehicle as these tokens cannot be used for broadcasting (bogus) safety messages.  The vehicle refreshes its pseudonym certificate for another time window $\tw$ by presenting a valid token to an RSU ($\pseudogen$ protocol); a feature of our system is that the refresh requires a single node (\ie an RSU), which makes it reasonable for vehicular environments with short-time network coverage.  In case of anomalies or misbehavior (\eg a compromise), a revocation protocol ($\revoke$) is run to report a vehicle to the backend and update corresponding revocation lists. Because our system uses short-lived pseudonym certificates, and it does not allow a vehicle to keep pseudonym certificates of future time windows, other vehicles do not need to keep track of revoked vehicles (\ie no need for a CRL);  the system only needs to revoke the tokens, and such a token revocation list $\TRL$ needs to reside at the RSUs (which do not have the network limitations as vehicles) to prevent  revoked vehicles from refreshing their pseudonym certificates.  Our system additionally makes use of the existing infrastructure for refreshing pseudonym certificates, which improves the system scalability.



% Roughly speaking, $\setup$ is only run once per vehicle to produce a long-term certificate. $\tokengen$ is run whenever a vehicle needs to get a list of authorization tokens (e.g., once a week, month, year ..etc) that allow it to request short-term pseudonym certificates. $\pseudogen$ is run whenever the vehicle needs to get a short-term pseudonym certificate that allows it to communicate anonymously with other vehicles.  $\revoke$ is invoked to revoke the privileges of a misbehaving vehicle to prevent it from participating in the system.  We begin with a high level discussion of each algorithm.

\paragraph{Subroutines}
We here describe the subroutines of our system briefly.


\begin{itemize}
    \item $\setup(\vk_v,\text{\att}, \sk_\B)${\bf :} it takes in a verification key $\vk_v$, an attestation $\att$,   and a signing key $\sk_\B$; it outputs a long-term certificate $\ltc_v$.
    \item $\tokengen(\sk_v, \ltc_v, Req, \sk_\B)${\bf :} it takes in a signature key $\sk_v$, a long-term certificate $\ltc_v$, a request $Req$ and a singing key $\sk_\B$; it outputs a token list  $\T$.
    \item $\pseudogen(t, \sk_{RSU}, \vk_\B)${\bf :} it takes in a token $t$, and signing and verification keys, $\sk_{RSU}, \vk_\B$, respectively; it outputs a pseudonym certificate $\pc$.
    \item $\revoke(\pc, \rep)${\bf :} it takes in a pseudonym certificate $\pc$ and a report $\rep$; it outputs an updated black list $\BL$ and a token revocation list $\TRL$. 
 \end{itemize}




\subsection{Security Goals}
We here informally describe the the desired security properties, which our design attains.
\begin{itemize}
    \item {\bf Message integrity and authenticity:} assert that the message is coming from a valid system participant without illegitimate alterations.
    \item {\bf Anonymity:} vehicle messages cannot be used to reveal a vehicle real identity.
     \item {\bf Short-term linkability:} messages from a single vehicle can be linked by other vehicles in a single time-window.
    \item {\bf Long-term unlinkability:} messages from a single vehicle cannot be linked by other vehicles, manufacturers, RSUs or the backend so as to prevent tracking vehicle routes.
    \item {\bf Physical location privacy:} the backend system cannot learn  physical location of vehicles in such a way that allows it to track vehicles' long-term driving routes.
    \item {\bf Traceability:} Only two separate components, namely the backend and an RSU, can jointly trace a vehicle real identity, if needed (\eg for revocation).
    \item {\bf Revocation:} misbehaving/compromised vehicles can be revoked from the system.
    \item {\bf Retrospective unlinkability:} misbehaving/compromised vehicles  messages can only be linked from the time of revocation/compromise on.
    \item {\bf Resistance against Sybil attacks:} a compromised vehicle does not allow an attacker to masquerade as multiple vehicles at the same time.
\end{itemize}

We assume an adversary $\calA$ can compromise vehicles or RSUs. We also assume multiple RSUs might collude to try to break any of the desired security properties.


















\section{Design Overview}

\subsection{Notations}
We here set some notations.  $x\leftarrow\$$ means $x$ is assigned a random value. $(\ek,\dk)$ denote a pair of asymmetric encryption and decryption keys, respectively. $(\sk,\vk)$ denote a pair of asymmetric signing and verification keys, respectively. $\ltc$, $\pc$ and $\ac$ denote long-term and pseudonym certificates, respectively, where $\{\ltc, \pc\}\leftarrow(\vk, \sigma)$ for $\sigma$ is a signature on $\vk$. $\st,\et$ denote  start and end times of a time window $\tw$, respectively. $\TF=\{\tw_1, \cdots, \tw_N\}$ denotes a list of unique time windows, where $\tw_{i+1}>\tw_i$.  $\T = \{t_1, \cdots, t_N\}$ denotes a list of tokens, where tokens $t_i,t_{i+1}\in\T$ are valid at time windows $\tw_i,\tw_{i+1}$, respectively. A token contains $t\leftarrow(\id, \tw, \sigma)$, where $\id$ is a token identity, and token's content $\tc\leftarrow(\id, \tw)$.   $\BL$ denotes a long-term certificate black list, which is local to the backend $\B$. $\TRL$ denotes a token revocation list, which is updated by the backend and distributed to RSUs. $\UTL$ denotes a local list of tokens that has been seen by an RSU. $\pt, \ct, \msg$ denote a plaintext, ciphertext and message, respectively. 

\subsection{System Model and Assumptions}
The system consists of a set of vehicles $\V$, a set of road-side units $\RSU$, the backend $\B$ and a set of manufacturers $\M$. 
% \silas{don't we also need a RSU backend?}
The goal of the system is to provide the vehicles $v\in\V$ with temporary, anonymous, authenticated certificates $-$ \emph{pseudonym certificates} $-$ which they will then use to authenticate their communications with other vehicles. 
% The reason they are anonymous and temporary is because we need to stop curious entities (e.g., vehicles, RSUs or even the backend system) from using vehicle's messages to track its long-term driving activities. In other words, the system needs to achieve the anonymity and long-term unlinkability properties, which become a challenge when designing such a system. Anonymity ensures that a vehicle real identity is not revealed as a result of its authenticated vehicle to vehicle (V2V) communications. Long-term unlinkability ensures that pseudonym certificates of a single vehicle used in V2V communications cannot be linked to the same vehicle. 
In a vehicular communication environment,  the assumption is that road-side units (RSUs) are always deployed across roads and highways, and connectivity with the backend is only available through them.  Because RSUs have a small network coverage area and might have intermittent connectivity with the backend (\eg consider a rural area where RSUs rely on wireless internet service providers, WISPs), vehicles often have short-time connectivity with RSUs (e.g., consider a vehicle driving on a highway) and have no frequent stable connectivity with the backend.
% To fix this issue, our system provides the infrastructure with the ability to instantly refresh pseudonym certificates for vehicles while still achieving anonymity and long-term unlinkability.

In our system, we assume the backend and RSUs are equipped with pairs of asymmetric encryption and decryption keys, $(\ek_\B,\dk_\B)$ and $(\ek_{RSU},\dk_{RSU})$ respectively. Also, the backend has a pair of asymmetric signing and verification keys $(\sk_\B,\vk_\B)$ and a self-signed certificate $\ltc_\B$ that is the root of trust in the system; this backend could be the Department of Motor Vehicles (DMV), Department of Transportation (DoT) ..etc. Each RSU has a pair of $(\sk_{RSU},\vk_{RSU})$ and a certificate $\ltc_{RSU}$ signed by the backend; this certificate allows an RSU to generate pseudonym certificates for vehicles. Each manufacturer also has a pair of $(\sk_{m},\vk_{m})$ and a certificate $\ltc_m$ signed by the backend; this certificate is used for attesting vehicle requests to get long-term certificates.  Communications between vehicles, RSUs and the backend always occur over a secure channel (\eg TLS). We also assume that all communications with the backend pass through a location obscurer proxy that conceals network addresses in order to hide the other party's physical location from the backend. 





\subsection{System Overview}
Our system consists of four algorithms (\setup, \tokengen, \pseudogen, \revoke). Roughly speaking, $\setup$ is only run once per vehicle to produce a long-term certificate. $\tokengen$ is run whenever a vehicle needs to get a list of authorization tokens (e.g., once a week, month, year ..etc) that allow it to request short-term pseudonym certificates. $\pseudogen$ is run whenever the vehicle needs to get a short-term pseudonym certificate that allows it to communicate anonymously with other vehicles.  $\revoke$ is invoked to revoke the privileges of a misbehaving vehicle to prevent it from participating in the system.  We begin with a high level discussion of each algorithm.


Our system consists of four algorithms (\setup, \tokengen, \pseudogen, \revoke). When a vehicle is about to be  used for the first time, it needs to go through a setup protocol $(\setup)$ to get a long-term certified identity (\ie long-term certificate); such certificates are the means that allows legitimate vehicles to authenticate themselves when communicating with the backend system. In order to improve passenger safety and road efficiency in a vehicular environment, vehicles are urged to share their road observations with nearby vehicles to allow for better driving decisions;   such observations need to be shared in an authenticated manner to prevent adversaries from degrading road efficiency or causing road accidents. Naively, a vehicle would authenticate such observations using its long term certificate and broadcast them to other vehicles. However, this proposes privacy concerns as the vehicle's messages carry its real identity; this could allow the backend, RSUs, manufacturers or other vehicles to collect such messages and track the vehicle's driving activities. Therefore, a vehicular communication system needs to anonymize vehicle identities; \emph{anonymity} ensures that a vehicle real identity is not revealed (to the backend, RSUs, manufacturers and other vehicles) as a result of its authenticated vehicle to vehicle (V2V) communications. While the backend could additionally, at $\setup$, provide a pseudonym identity for anonymous V2V communications,  it still can identify  messages of a single vehicle since the backend knows the corresponding long term and pseudonym identities  (\ie no anonymity from the backend). One way to overcome this issue is to divide this process into two tasks and assign them to two nodes within the system (\ie two nodes at the backend), where one does long-term certificate verification and the other creates pseudonym certificates; 
% this solution introduces other issues as will be discussed below.

While anonymity conceals a vehicle's identity, it still does not conceal its driving activities; this provides valuable information for eavesdroppers that allows  route tracking (which might eventually be linked to the vehicle, say if a vehicle is compromised). One way to address this issue is to allow the vehicles to have multiple pseudonym identities (\eg multiple pseudonym certificates, group signature schemes ..etc); however, it is important to note that this same approach could allow for masquerading as multiple vehicles (\ie a Sybil attack) if multiple pseudonym identities could be used at the same time window. One seemingly proper way to utilize this approach is to make vehicles use a pseudonym certificate for a single message communication only; while this approach achieves optimal unlinkability, this is not desirable in vehicular environments.  Linking messages of a single anonymous vehicle for a period of time (\eg several minutes) is important as it enables other vehicles to make critical driving decisions; for example, it helps connected vehicles to use broadcast messages of other vehicles to avoid crashes as a result of unexpected behavior of other surrounding vehicles (\eg critical connected vehicle applications: forward collision warning FCW, Emergency Electronic Brake Light EEBL ...etc).      Therefore, a vehicular communication system only needs to hide the \emph{long-term} driving activities of a single vehicle in order to prevent tracking; \emph{long-term unlinkability} ensures that pseudonym certificates of a single vehicle used in V2V communications cannot be linked to the same vehicle. One way to achieve this property is to pre-load a vehicle with a set of consecutively valid independent pseudonym certificates (\eg a year worth of certificates). However, in case of a vehicle compromise, the attacker is able to participate in the system till the end of the year; certificate revocation lists (CRLs) can be used to mitigate this attack, but they grow large over time and it becomes too large to download them especially for vehicles with short-time network connectivity. Another solution is to make vehicles periodically refresh their pseudonym certificates whenever they get connectivity (\ie be in an RSU vicinity), but this is not reasonable in vehicular environments due to intermittent connectivity and long network latency with the backend.

In order to design a system that avoids all the aformentioined issues, our system delegates the pseudonym certificate generation task completely to the infrastructure. A vehicle runs a token generation protocol ($\tokengen$) which allows it to get a list of tokens $\T = \{t_1,\cdots,t_N\}$; each token $t_i$ serves as an authorization from the backend that the vehicle can use to refresh a pseudonym certificate at time window $\tw_i$. Note that this is the only process that requires the vehicle to communicate with the backend system, and it takes place only one time for some time period (\eg once a year). Most importantly, tokens have no values that can be used to reveal vehicles' identities. This limits the attacker ability when compromising a vehicle as these tokens cannot be used for broadcasting (bogus) safety messages.  The vehicle refreshes its pseudonym certificate for another time window $\tw$ by presenting a valid token to an RSU ($\pseudogen$ protocol); a feature of our system is that the refresh requires a single node (\ie an RSU), which makes it reasonable for vehicular environments with short-time network coverage.  In case of anomalies or misbehavior (\eg a compromise), a revocation protocol ($\revoke$) is run to report a vehicle to the backend and update corresponding revocation lists. Because our system uses short-lived pseudonym certificates, and it does not allow a vehicle to keep pseudonym certificates of future time windows, other vehicles do not need to keep track of revoked vehicles (\ie no need for a CRL);  the system only needs to revoke the tokens, and such a token revocation list $\TRL$ needs to reside at the RSUs (which do not have the network limitations as vehicles) to prevent  revoked vehicles from refreshing their pseudonym certificates.  Our system additionally makes use of the existing infrastructure for refreshing pseudonym certificates, which improves the system scalability.



% Roughly speaking, $\setup$ is only run once per vehicle to produce a long-term certificate. $\tokengen$ is run whenever a vehicle needs to get a list of authorization tokens (e.g., once a week, month, year ..etc) that allow it to request short-term pseudonym certificates. $\pseudogen$ is run whenever the vehicle needs to get a short-term pseudonym certificate that allows it to communicate anonymously with other vehicles.  $\revoke$ is invoked to revoke the privileges of a misbehaving vehicle to prevent it from participating in the system.  We begin with a high level discussion of each algorithm.

\paragraph{Subroutines}
We here describe the subroutines of our system briefly.


\begin{itemize}
    \item $\setup(\vk_v,\text{\att}, \sk_\B)${\bf :} it takes in a verification key $\vk_v$, an attestation $\att$,   and a signing key $\sk_\B$; it outputs a long-term certificate $\ltc_v$.
    \item $\tokengen(\sk_v, \ltc_v, Req, \sk_\B)${\bf :} it takes in a signature key $\sk_v$, a long-term certificate $\ltc_v$, a request $Req$ and a singing key $\sk_\B$; it outputs a token list  $\T$.
    \item $\pseudogen(t, \sk_{RSU}, \vk_\B)${\bf :} it takes in a token $t$, and signing and verification keys, $\sk_{RSU}, \vk_\B$, respectively; it outputs a pseudonym certificate $\pc$.
    \item $\revoke(\pc, \rep)${\bf :} it takes in a pseudonym certificate $\pc$ and a report $\rep$; it outputs an updated black list $\BL$ and a token revocation list $\TRL$. 
 \end{itemize}




\subsection{Security Goals}
We here informally describe the the desired security properties, which our design attains.
\begin{itemize}
    \item {\bf Message integrity and authenticity:} assert that the message is coming from a valid system participant without illegitimate alterations.
    \item {\bf Anonymity:} vehicle messages cannot be used to reveal a vehicle real identity.
     \item {\bf Short-term linkability:} messages from a single vehicle can be linked by other vehicles in a single time-window.
    \item {\bf Long-term unlinkability:} messages from a single vehicle cannot be linked by other vehicles, manufacturers, RSUs or the backend so as to prevent tracking vehicle routes.
    \item {\bf Physical location privacy:} the backend system cannot learn  physical location of vehicles in such a way that allows it to track vehicles' long-term driving routes.
    \item {\bf Traceability:} Only two separate components, namely the backend and an RSU, can jointly trace a vehicle real identity, if needed (\eg for revocation).
    \item {\bf Revocation:} misbehaving/compromised vehicles can be revoked from the system.
    \item {\bf Retrospective unlinkability:} misbehaving/compromised vehicles  messages can only be linked from the time of revocation/compromise on.
    \item {\bf Resistance against Sybil attacks:} a compromised vehicle does not allow an attacker to masquerade as multiple vehicles at the same time.
\end{itemize}

We assume an adversary $\calA$ can compromise vehicles or RSUs. We also assume multiple RSUs might collude to try to break any of the desired security properties.





% \begin{itemize}
%     \item $\setup(1^n)${\bf :} a new vehicle $v\in V$ picks an identity $\id$; the backend system outputs $\ltc_v = (\id, \sigma_{id})$ and performs $\LTC := \ltc_v \cup \LTC$; this algorithm is performed once per vehicle; $v$ keeps the tuple $\ltc_v$; initially, $\LTC = \emptyset$, $\BL = \emptyset$ and $\TRL = \emptyset$.
%     \item $\tokengen(\ltc_v, \st_i, \et_i)${\bf :} it takes in a start time $\st_i$ and end time $\et_i$ for the token list $\T_i$; the backend verifies $\ltc_v\in\LTC$, $\ltc_v\notin\BL$, $\st_i > \et_{i-1}$ and produces  $\T_i := \{t_1, \cdots, t_N$\} where $N = et_i - st_i/\tw$.
%     \item $\pseudogen(t_j)${\bf :} $v$ chooses a pseudonym identity $\pid$; a road-side unit $r\in\RSU$ verifies $t_j\notin\TRL$ and outputs $\pc_v := (\pid, \sigma_{pid})$; $r$ keeps the tuple $(t_j, \pc_v)$.
%     \item $\revoke(\pc_v)${\bf :} the backend finds $r\in\RSU$ and gets the corresponding token $t_j\in\T_i^v$; it also uses $t_j$ to find the corresponding $\ltc_v$; it performs $\BL :=  \BL \cup \ltc_v$ and $\TRL = \TRL \cup \{t_j,\cdots,t_N\}$; $\forall r\in\RSU$,   $r$ gets the updated $\TRL$.
%  \end{itemize}




==> problem_def.tex <==

\newcommand{\RSU}{{\sf RSU}}
\newcommand{\V}{{\sf V}}
\newcommand{\B}{{\sf B}}
\newcommand{\ltc}{{\sf ltc}}


\section{Problem Definition}

% \subsection{Entities}
% The system consists of a set of vehicles $\V$, road-side units $\RSU$  and the backend components $\B$. $v\in\V$ is the main component that utilizes the system by anonymously broadcasting messages about the surrounding status of the road to other vehicles $v'\in V'\subset\V$ to help them make better driving decisions. $r\in\RSU$ is main point that allows communication between $v\in\V$ and $b\in\B$ and also helps in creating pseudonym identities for $v$. The backend set $\B$ has the following components:
% \begin{itemize}
%     \item Root Certificate Authority (Root CA): this is the root of  trust (top of hierarchy) in the whole system and is responsible for extending administrative  privileges to other nodes (e.g., creating certificates). Root CA has a self-signed certificate and is typically offline to protect it from attacks due to its critical role. 
%     \item Intermediate Certificate Authority (Intermediate CA): it is the second node in the chain, has a certificate from the Root CA and is responsible for creating certificates to components $c\in\B$, $r\in\RSU$ as well as long term certificates $\ltc$ and tokens for $v\in\V$. 
%     \item Device Configuration Manage (DCM): attests to the request that a vehicle is eligible for a long-term certificate $\ltc$.
%     \item Misbehavior Authority (MA): 
% \end{itemize}

\subsection{System Model and Assumptions}
The IoV system involves vehicles, road-side units (RSUs) and the backend system.


\subsection{Requirements for Vehicular Key Management System}
\begin{itemize}
    \item {\bf Message integrity and authenticity:} assert that the message is coming from a valid system participant without illegitimate alterations.
    \item {\bf Anonymity:} messages cannot be used to reveal a vehicle real identity.
     \item {\bf Short-term linkability:} messages from a single vehicle can be linked by other vehicles in a single time-window or area.
    \item {\bf Long-term unlinkability:} messages from a single vehicle cannot be linked by other vehicles or the main system (including the backend and road side units, RSUs) so as to prevent tracking vehicle routes.
    \item {\bf Physical location privacy:} the backend system cannot learn  physical location of vehicles in such a way that allows it to track vehicles' long-term driving routes.
    \item {\bf Traceability:} Only two separate components of the main system  together can trace a vehicle real identity, if needed (\eg for revocation).
    \item {\bf Revocation:} misbehaving vehicles can be revoked from the system.
    \item {\bf Retrospective unlinkability:} misbehaving/compromised vehicles  messages can only be linked from the time of revocation/compromise on.
    \item {\bf Resistance against Sybil attacks:} a compromised vehicle does not allow an attacker to masquerade as multiple vehicles at the same time.
\end{itemize}
\hfill

The following explains the requirements to achieve each of the above security properties. 

\begin{itemize}
    \item {\bf Message integrity and authenticity:}
        \begin{itemize}
            \item All message exchanges must be digitally signed.
        \end{itemize}
    \item {\bf Anonymity:} 
    \begin{itemize}
        \item Messages/identities broadcast must not indicate a real vehicle identity.
        \item No single entity in the main system (\eg backend/RSU ..etc) can know both the real vehicle identity and its pseudonym identity.
    \end{itemize}
    \item {\bf Short-term linkability:} 
    \begin{itemize}
        \item A vehicle must reuse the same pseudonym identity for a short-time interval or in an area when broadcasting messages.
    \end{itemize}
     \item {\bf Long-term unlinkability:} 
    \begin{itemize}
        \item Each pseudonym identity of a single vehicle must look random and independent.
        \item No single entity in the main system (\eg backend/RSU ..etc) can know that two or more pseudonym identities belong to a single (unknown) vehicle.
    \end{itemize}
     \item {\bf Physical location privacy:} 
    \begin{itemize}
        \item Each request must directly/indirectly indicate no physical location information (\eg network addresses).
        
    \end{itemize}
    \item {\bf Traceability:} 
    \begin{itemize}
        \item The main system needs to make sure it is provided proof of vehicle real identity before allowing the vehicle to participate.
    \end{itemize}
      \item {\bf Revocation:} 
    \begin{itemize}
        \item The main system needs to maintain, update and distribute revocation lists of misbehaving vehicles to the backend and RSUs to prevent revoked vehicles from participating.
         
    \end{itemize}
     \item {\bf Retrospective unlinkability:} 
    \begin{itemize}
        \item Pseudonym identities of a single vehicle need to be random and independent so that compromised/revoked pseudonym identities cannot be linked to previous pseudonym identities of the same vehicle when it was not compromised/revoked. 
    \end{itemize}
    \item {\bf Resistance against Sybil attacks:} 
        \begin{itemize}
            \item The vehicle must not be issued two or more pseudonym identities that are valid at the same time.
        \end{itemize}
 
\end{itemize}
\subsection{Threat Model}

==> smcsdetails.tex <==

\section{A Survey of SCMS}
\label{sec:scmsdetails}
% \silas{Three things:
% \begin{enumerate}
%     \item This section needs some discussion here to introduce and summarize the rest of the section.  Maybe say something like "In this section we expand on our description of SCMS from Section~\ref{sec:scmsbackground} by describing the interactions between the system elements in more detail."
    
%     \item There should be a small paragraph reminding the reader what's going on: who are the parties, what is the goal of the system (there's a paragraph you can copy from in Section~\ref{sec:scmsbackground}).  Right now this section just launches directly into dense crypto.  It feels too abrupt to me...
    
%     \item If you're going to include $g^x$ notation then you need to introduce this in the crypto prelims section.  You could probably pull from the mergeable signatures paper.
% \end{enumerate}
% }


SCMS (Figure \ref{fig:scms overview}) is the official VPKI system adopted by the US DoT and therefore in this section we will provide a more detailed description for the interested readers on how the SCMS works under-the-hood.

\subsection{Overview}

Before a vehicle participates in the SCMS, it must obtain a long-term certificate, called Enrollment Certificate (EC), signed by an Enrollment Certification Authority (ECA). All messages sent by the vehicle to the SCMS must be signed by its EC. Once a vehicle owns an EC (which only happens once for each new vehicle or vehicle ownership transfer), the vehicle can request multiple Pseudonym Certificates (PC) from an SCMS entity called Pseudonym Certification Authority (PCA). The PCs are then used to communicate securely and \emph{anonymously} with other vehicles while the sending vehicle keeps swapping between PCs (e.g. every 5 minutes) to preserve \emph{unlinkability}. The suggested SCMS parameters allow a vehicle to have 20 to 40 PCs that are simultaneously valid for one week. All PC requests are sent to an SCMS entity called Registration Authority (RA) that validates, processes, and forwards requests for PCs to the PCA. 

The division-of-labor between PCA and RA is to preserve the unlinkability and anonymity of vehicles. Furthermore, to preserve the vehicles' location anonymity, all vehicles' messages to the SCMS are tunneled through an SCMS gateway called Location Obscurer Proxy (LOP) which has the role of obscuring the vehicle's location (i.e. IP address) by sending the vehicle's messages on its behalf to the desired SCMS destination server. In case of a vehicle misbehavior incident, the Misbehavior Authority (MA) is the SCMS entity responsible of initiating the revocation process among the other SCMS entities with the support of Linkage Authority 1 (LA1) and Linkage Authority 2 (LA2). LA1 and LA2 store a hash chain for each vehicle where each value in the hash can be used by the MA to reveal a vehicle identity. The division-of-labor between two Linkage Authorities is implemented to prevent a single authority from unlawfully revealing the identities of vehicles.

\subsection{PC Provisioning}
\label{sub:pc_provisioning}
When a vehicle wants to obtain a PC, it sends a PC request signed by its corresponding EC to the SCMS backend system via an RSU. First, the vehicle creates a PC public/private keypair $(g^x, x)$ and a session public/private keypair $(g^y, y)$. Then, the vehicle creates a PC request, attaches $g^x$ and $g^y$, signs it with its EC, then sends it to the backend system. The request is then relayed from the RSU to the RA via the LOP to hide the vehicle's location. Then for each PC request, the RA creates two sets of 20 random numbers \cut{$r_{i} \in $}$\{r_{1},\cdots, r_{20}\}$ and \cut{$r'_{j} \in $}$\{r'_{1},\cdots, r'_{20}\}$ (assuming the SCMS is configured to generate 20 PCs per request). The RA then raises $g^x$ to each $r_{i}$ and $g^y$ to each $r'_{i}$ for all ${i=1, \cdots, 20}$, creating two sets of 20 different public keys each, $\{g^{x.r_{i}}\}_i$ and $\{g^{y.r'_{i}}\}_i$; this process is known as Butterfly Key Expansion and its main purpose is to offload the creation of the 20 public keys to the RA (without knowledge of corresponding private keys) which reduces vehicle uplink bandwidth. After that, the RA sends each pair of ($g^{x.r_{i}}, g^{y.r'_{i}}$) to the PCA. 

Note that to preserve the unlinkability requirement, the RA shuffles between the pairs from different vehicles' requests before sending them to the PCA. This prevents the PCA from linking a group of keypairs (and ultimately PCs) to the same vehicle since PCA (according to the discrete log assumption) cannot distinguish if $g^{x.r_{i}},g^{x.r_{j}}$ are generated from the same PC request. The PCA then creates a random number $\hat r_{i}$ for each $g^{x.r_{i}}$ and raises it to that random number and signs the newly created PC public key using the PCA's private key, creating a PC$ = (g^{x.r_{i}.\hat r_{i}}, \sigma)$. The process of raising $g^{x.r_{i}}$ to a new random number $\hat r_{i}$ by the PCA is done to prevent the RA from linking multiple PCs to the same vehicle (preserving unlinkability) since the RA is the SCMS entity who performed the Butterfly Key Expansion process. It also prevents the RA from linking a PC to its corresponding EC (preserving anonymity) since it knows who is the requesting vehicle. After that, the PCA encrypts $\ct = $(PC, $\hat r_{i}$) using its paired $g^{y.r'_{i}}$ (which is originally received from the RA) and sends it back to the RA. Finally, the RA sends the newly signed 20 PCs to the requesting vehicle by relying  $\{\ct, r_{i}, r'_{i}\}$ over a secure channel (\eg TLS).

Note that the PCA and RA keep a \emph{request reference number} for each keypair in order for the RA to know which signed PC to send to which vehicle without the need of looking into the encrypted content of $\ct$. Upon receiving the response from the RA, the vehicle computes the expanded private key of each $g^{y.r'_{i}}$ as $y.r'_{i}$ and decrypt the PCA messages. It then computes the expanded private keys of each PC, $g^{x.r_{i}.\hat r_{i}}$ as $x.r_{i}.\hat r_{i}$.

\subsection{Enrollment \& PC Revocation}
\label{sub:scms_revocation}

\vskip3mm \noindent\textbf{Creating Linkability:} If a vehicle misbehaves, the SCMS should be able to link the vehicle's PC to its EC for revocation and accountability. 
% The PC provisioning process described in the previous section provides complete unlinkability even if all SCMS entities cooperate together (which is undesirable).
Naively, all non-expired PCs of a single revoked vehicle are added to the pseudonym certificate revocation list (PCRL) upon revocation. However, the PCRL size becomes extremely large and bandwidth consuming since SCMS generates a large number of PCs (\eg 20 per vehicle) that are valid for a long time (\eg a week).



\begin{figure}[t]
% \vspace{-5pt}
\centering 
\includegraphics[width=\linewidth,keepaspectratio]{Images/SCMS_overview_4.png}
% \vspace{-6pt}
\caption{SCMS Architecture Overview~\cite{CV2019USDOT}.}
% \ahmed{Is this your diagram?} \abdulrahman{this diagram is brought from the SCMS conference paper}
\label{fig:scms overview}
% \vspace{-12pt}
\end{figure}



In order to have a fixed number of entries (namely one entry per revoked vehicle) regardless of the number of revoked PCs owned by the vehicle, SCMS links all PCs of a single vehicle using a hash chain of PC linkage information called a Linkage Value $LV$ (acts like a PC ID) and is added to each $PC$ created by the PCA which is then used by the MA to revoke the misbehaving vehicle with the help of other SCMS entities.

To create the $LV$, two SCMS entities are responsible for this task, called Linkage Authority 1 ($LA_{1}$) and Linkage Authority 2 ($LA_{2}$). For each newly created $EC$, each $LA$ independently creates and assigns a random number for that $EC$ called Linkage Seed 0 ($LS_{0}$) which will be used to create a hash chain of Linkage Seeds $LS_{i}$ such that $LS_{i+1} = H(LS_{i})$. Each $LS_{i}$ acts as a reference value for a batch of 20 $PCs$. The $LS_{i}$ is then used to create 20 different values called Prelinkage Values $PV_{j} \in (PV_{1},...,PV_{20})$ using an AES function such as $PV_{j} = \enc_{LS_{i}} (j||LA_{ID})$ where $LA_{ID}$ is the ID of the $LA$ which is used to prevent the chance of having the two $LAs$ randomly choose the same $LS_{0}$ seed for the same vehicle. Finally, each $PV_{j}$ from $LA_{1}$ and $LA_{2}$ for a given batch $LS_{i}$ are XORed together creating $LV_{i,j}$ ($LV$ for PC $j$ from batch number $i$). Notice that the creation of a single $LV$ is divided between two $LAs$ to prevent a single LA from linking multiple $PCs$ by simply looking at their $LVs$. Also, the PCA cannot retrieve the two corresponding $LS_i$ given the two $PV_j$ only because it does not know the AES key (\ie $LS_i$). Furthermore, the XORing operation of the two $PV_{j}$ is done by the $PCA$ during the $PC$ creation process. 

Note that since the PCA does not know the EC of the requesting vehicle, the LAs cannot determine from which $LS_{0}$ seed the $PV$ should be derived from since the PCA cannot provide the EC to them. Therefore, the $PV$ request is done by the RA on behalf of PCA during the key expansion process (since RA is the entity who knows the EC of the requesting vehicle and the batch number $i$) and passes it to the PCA. Furthermore, to prevent the RA from linking PCs to the same vehicle via their $LVs$ (by XORing its $PVs$), LAs encrypt the $PVs$ with the PCA's public key before passing them to the RA.

\vskip3mm \noindent\textbf{Revoking a Misbehaving Vehicle's Certificate:} Once a vehicle is determined to be misbehaving, the MA contacts the PCA and requests the \emph{PC request reference number} between the PCA and the RA that was used to create the misbehaving PC. Based on reference number, the MA instructs the RA to add the EC of the vehicle who requested the PC, to an SCMS internal blacklist (\BL) in order to prevent future PC provisioning requests from the misbehaving vehicle. Then the MA (with the help of RA) instructs the two LAs to reveal their $LS_{i}$ for the blacklisted EC (via EC initial seed $LS_{0}$) for a given batch $i$. Assuming the SCMS is configured to allow a vehicle to have 20 $PCs$ every week, each $LS_{i}$ represents the linkage seed of week $i$ for a vehicle. In other words, based on the validity time of a given PC, the batch number is inferred from the week number. After that, the two LAs add the $LS_{i}$ of the misbehaving vehicle to a public PCRL. Once the two $LS_{i}$ are made public, any vehicle can compute all subsequent $LS_{i+1}$, derive the $PV$ for week $i+1$, and XOR the $LVs$ of the misbehaving vehicle for all subsequent weeks until the vehicle's EC expiration date (or simply until the end of the current week since the misbehaving vehicle is blacklisted from any future PCs).



==> system_optimization.tex <==
\section{\name\ Optimization}
In this section, we introduce a mechanism that allows linking tokens of a single vehicle secretly; this allows for significant reduction in storage requirements of such tokens as well as the size of token blacklist ($\TRL$) when  vehicles are revoked.

\vskip 3mm\noindent{\bf Linked Tokens via Hash Chains.} We propose a novel approach that allows for generating token ids for a single vehicle $v$ that look random and independent   but can still be selectively linked using a secret that is  kept at $\CA$ only. Particularly, it provides two advantages: 1) It allows $\CA$ to publish a single $\tau$ id (and a secret) per revoked $v$, which can significantly reduce token blacklist (\TRL) bandwidth requirements since the $\TRL$ size becomes based on the number of revoked vehicles rather than revoked tokens. 2) The $\CA$ can keep a single $\tau$ id (and a secret) at any time window and derive the ids of tokens of future time intervals; the same approach can also be utilized by $\rsu\in\RSU$ when tokens are revoked. This can significantly reduce the storage requirements of keeping such token ids at $\CA$ and $\rsu$. 

Before explaining our hash chain approach (Figure~\ref{fig:New Hash Chain}), we first discuss the intuition behind it.  The approach utilizes hash chains because each hash value of theirs look random and thus can be used as a $\tau$ id. However, since the hash function $H$ is public, $\rsu$ can determine if two hashes $x_i, x_{j}$ belong to the same chain by using one to derive the other using $H$, which violates unlinkability. To fix this issue,  $\CA$ uses a per vehicle secret $r$ as part of the $H$ input  to traverse the $\tau$ id hash chain of $v$; thus, $\rsu$ is unable to link $\tau$ ids without knowledge of $r$ due to the inversion hardness assumption of $H$. Additionally,  upon revocation and revealing the secret $r$,
% that allows $\rsu$ to derive other token ids of $v$, 
our mechanism needs to preserve unlinkability of $v$ before it was revoked (\eg protect privacy of a stolen $v$). To achieve this property, the per vehicle secret $r$ is also constructed as another hash chain as shown in Figure~\ref{fig:New Hash Chain}; thus, when $v$ is revoked at a time interval, only corresponding hash values from both hash chains are revealed,  which only allow $\rsu$ to derive current and future revoked tokens of $v$. 

Our hash chain mechanism works as follows; At vehicle $\setup$,  $\CA$ picks two random values, $x_0$,$r_0$, called heads. Upon executing $\pseudogen$, $\CA$ uses $H$ and the heads $x_0$,$r_0$ to create two hash chains of length $N+1$, where $N$ is the number of tokens generated as a result of this request; the next $\pseudogen$ request heads become $x_N$,$r_N$. In the hash chain of secrets (\ie $r_0,\cdots,r_N$), at the $i^{th}$ position, the value is calculated by $H(r_{i-1})$. The second hash chain, which produces the $\tau$ ids, makes use of the values from the first chain. Specifically, the value at the $i^{th}$ position is calculated by applying $H(x_{i-1} || r_{i-1})$.  Whenever a malicious vehicle is detected, then the remaining tokens are revoked by publishing the corresponding input values to the current token $x_i$ being revoked, that is, $(x_{i-1}, r_{i-1})$. With this, the $\rsu$ will be able to invalidate the other remaining tokens acquired by the revoked $v$, which allows $\rsu$ to detect and refuse providing new PCs to revoked vehicles. 
% Due to the inversion hardness assumption of $H$, $\rsu$ cannot link the revoked tokens with previously used valid tokens by $v$ and hence linkability is not possible..



\begin{figure}[t]
% \vspace{-0pt}
\centering
\includegraphics[width=\linewidth,keepaspectratio]{Images/new_hash_chain.png}
% \vspace{-0pt}
\caption{Our new hash chain mechanism.}
\label{fig:New Hash Chain}
% \vspace{-0pt}
\end{figure}

